$\varphi$-Calculus: Object-Oriented Formalism

Object-oriented programming (OOP) is one of the most popular paradigms used for building software systems. However, despite its industrial and academic popularity, OOP is still missing a formal apparatus similar to $\lambda$-calculus, which functional programming is based on. A number of attempts were made to formalize OOP, but none of them managed to cover all the features available in modern OO programming languages, such as C++ or Java. We have made yet another attempt and created $\varphi$-calculus. This paper does not demonstrate the practical use or effect of $\varphi$-calculus but merely explains it.

==> _eolang/paper/00E4E17B47A2A768DDD3F4CF912709D7-58-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 47 chars in the input: _eolang/paper/00E4E17B47A2A768DDD3F4CF912709D7-58-phiq.tex
% ---
%  e ( \tau _1 -> e_1 , \tau _2 -> e_2 , \dots ) 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(e \phiTerminal{(} \tau _1 \mathbin{\phiTerminal{\mapsto}} e_1 \phiTerminal{,}\; \tau _2 \mathbin{\phiTerminal{\mapsto}} e_2 \phiTerminal{,}\; \dots \phiTerminal{)}\)\endinput

==> _eolang/paper/00E4E17B47A2A768DDD3F4CF912709D7-58-phiq.tex <==
 e ( \tau _1 -> e_1 , \tau _2 -> e_2 , \dots ) 

==> _eolang/paper/016F57FCA53FAB4B24F285C67A4D20AF-6-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 39 chars in the input: _eolang/paper/016F57FCA53FAB4B24F285C67A4D20AF-6-phiq.tex
% ---
%  \phinoContextualize { e }{ k }{ n_3 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoContextualize { e }{ k }{ n_3 }\)\endinput

==> _eolang/paper/016F57FCA53FAB4B24F285C67A4D20AF-6-phiq.tex <==
 \phinoContextualize { e }{ k }{ n_3 } 

==> _eolang/paper/02DE7875D0871CF7B9DDEDDCDD173E2A-153-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 5 chars in the input: _eolang/paper/02DE7875D0871CF7B9DDEDDCDD173E2A-153-phiq.tex
% ---
% b.|x|
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(b\phiTerminal{.}\textnormal{\texttt{x}}{}\)\endinput

==> _eolang/paper/02DE7875D0871CF7B9DDEDDCDD173E2A-153-phiq.tex <==
b.|x|

==> _eolang/paper/02FDF4DA1A93B6B3434C3703A662C5FC-70-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 28 chars in the input: _eolang/paper/02FDF4DA1A93B6B3434C3703A662C5FC-70-phiq.tex
% ---
% [[ |a| -> e_1, |b| -> e_2 ]]
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\llbracket} \textnormal{\texttt{a}}{} \mathbin{\phiTerminal{\mapsto}} e_1\phiTerminal{,}\; \textnormal{\texttt{b}}{} \mathbin{\phiTerminal{\mapsto}} e_2 \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/02FDF4DA1A93B6B3434C3703A662C5FC-70-phiq.tex <==
[[ |a| -> e_1, |b| -> e_2 ]]

==> _eolang/paper/03677F305F3527C1E6C144EF8305F789-67-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 17 chars in the input: _eolang/paper/03677F305F3527C1E6C144EF8305F789-67-phiq.tex
% ---
%  [[ \tau -> e ]] 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\llbracket} \tau \mathbin{\phiTerminal{\mapsto}} e \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/03677F305F3527C1E6C144EF8305F789-67-phiq.tex <==
 [[ \tau -> e ]] 

==> _eolang/paper/0466CCE5A24492DB239551A4DDEF3B86-253-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 104 chars in the input: _eolang/paper/0466CCE5A24492DB239551A4DDEF3B86-253-phiquation.tex
% ---
% \phinoDataize{n_1}{e}{s_1}{\delta}{s_2} \quad\text{and}\quad \phinoDataize{n_2}{e}{s_1}{\delta}{s_2}{.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
\phinoDataize{n_1}{e}{s_1}{\delta}{s_2} \quad\text{and}\quad \phinoDataize{n_2}{e}{s_1}{\delta}{s_2}{.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/0466CCE5A24492DB239551A4DDEF3B86-253-phiquation.tex <==
\phinoDataize{n_1}{e}{s_1}{\delta}{s_2} \quad\text{and}\quad \phinoDataize{n_2}{e}{s_1}{\delta}{s_2}{.}


==> _eolang/paper/08677AD1AFBEDA84BE4568EE567DC795-90-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1038 chars in the input: _eolang/paper/08677AD1AFBEDA84BE4568EE567DC795-90-phiquation.tex
% ---
% [[ |x| -> \phinoMeet{basic-n:1}{ \phiTerminal{\rho} . |k| . \phiTerminal{\rho} . |t| : |t| }, |k| -> [[]], |t| -> [[]] ]] . |x| . |t| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize \phinoAgain{basic-n:1} ( \phiTerminal{\rho} -> [[ |x| -> \phinoAgain{basic-n:1}, |k| -> [[]], |t| -> [[]] ]] ) . |t| \phiNormalize[\nameref{r:skip}]
%   \phiNormalize \phinoAgain{basic-n:1} . |t| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize [[]] . \phiTerminal{\rho} . |k| . \phiTerminal{\rho} . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-n:1} ) \phiNormalize[\nameref{r:norho}]
%   \phiNormalize T . |k| . \phiTerminal{\rho} . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-n:1} ) \phiNormalize[\nameref{r:dd}]
%   \phiNormalize T . \phiTerminal{\rho} . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-n:1} ) \phiNormalize[\nameref{r:dd}]
%   \phiNormalize T . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-n:1} ) \phiNormalize[\nameref{r:dd}]
%   \phiNormalize T ( \phiTerminal{\rho} -> \phinoAgain{basic-n:1} ) \phiNormalize[\nameref{r:dc}]
%   \phiNormalize T{.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phinoMeet{basic-n:1}{ \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{k}}{} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{t}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} }\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}}\phiTerminal{,}\; \textnormal{\texttt{t}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phinoAgain{basic-n:1} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-n:1}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}}\phiTerminal{,}\; \textnormal{\texttt{t}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}} \phiTerminal{)} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiNormalize[\nameref{r:skip}]\phiEOL{}
& \quad{}\phiNormalize \phinoAgain{basic-n:1} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{k}}{} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-n:1} \phiTerminal{)} \phiNormalize[\nameref{r:norho}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}} \phiTerminal{.} \textnormal{\texttt{k}}{} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-n:1} \phiTerminal{)} \phiNormalize[\nameref{r:dd}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-n:1} \phiTerminal{)} \phiNormalize[\nameref{r:dd}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-n:1} \phiTerminal{)} \phiNormalize[\nameref{r:dd}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-n:1} \phiTerminal{)} \phiNormalize[\nameref{r:dc}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}}{.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/08677AD1AFBEDA84BE4568EE567DC795-90-phiquation.tex <==
[[ |x| -> \phinoMeet{basic-n:1}{ \phiTerminal{\rho} . |k| . \phiTerminal{\rho} . |t| : |t| }, |k| -> [[]], |t| -> [[]] ]] . |x| . |t| \phiNormalize[\nameref{r:dot}]
  \phiNormalize \phinoAgain{basic-n:1} ( \phiTerminal{\rho} -> [[ |x| -> \phinoAgain{basic-n:1}, |k| -> [[]], |t| -> [[]] ]] ) . |t| \phiNormalize[\nameref{r:skip}]
  \phiNormalize \phinoAgain{basic-n:1} . |t| \phiNormalize[\nameref{r:dot}]
  \phiNormalize [[]] . \phiTerminal{\rho} . |k| . \phiTerminal{\rho} . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-n:1} ) \phiNormalize[\nameref{r:norho}]
  \phiNormalize T . |k| . \phiTerminal{\rho} . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-n:1} ) \phiNormalize[\nameref{r:dd}]
  \phiNormalize T . \phiTerminal{\rho} . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-n:1} ) \phiNormalize[\nameref{r:dd}]
  \phiNormalize T . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-n:1} ) \phiNormalize[\nameref{r:dd}]
  \phiNormalize T ( \phiTerminal{\rho} -> \phinoAgain{basic-n:1} ) \phiNormalize[\nameref{r:dc}]
  \phiNormalize T{.}


==> _eolang/paper/08D31E7151E7C8E69A365552E6C279F0-43-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 54 chars in the input: _eolang/paper/08D31E7151E7C8E69A365552E6C279F0-43-phiq.tex
% ---
%  \phinoEvaluate { [[ B ]] }{ e }{ s_1 }{ n_1 }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoEvaluate { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} }{ e }{ s_1 }{ n_1 }{ s_2 }\)\endinput

==> _eolang/paper/08D31E7151E7C8E69A365552E6C279F0-43-phiq.tex <==
 \phinoEvaluate { [[ B ]] }{ e }{ s_1 }{ n_1 }{ s_2 } 

==> _eolang/paper/09C869548D5B0278E1BAA923C6F3945C-84-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 34 chars in the input: _eolang/paper/09C869548D5B0278E1BAA923C6F3945C-84-phiquation.tex
% ---
% [[ |x| -> [[ D> |00-2A| ]] ]] {.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{00-2A}}{} \phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}} {.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/09C869548D5B0278E1BAA923C6F3945C-84-phiquation.tex <==
[[ |x| -> [[ D> |00-2A| ]] ]] {.}


==> _eolang/paper/0BB4ABAA7A52EC9FFC0683F5B31F8337-89-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 76 chars in the input: _eolang/paper/0BB4ABAA7A52EC9FFC0683F5B31F8337-89-phiq.tex
% ---
%   Q.|number| ( @ -> Q.|bytes| ( @ -> [[ D> |FF-F0-00-00-00-00-00-00| ]] ) ) 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{number}}{} \phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}}  \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{bytes}}{} \phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{FF-F0-00-00-00-00-00-00}}{} \phiTerminal{\rrbracket{}} \phiTerminal{)} \phiTerminal{)}\)\endinput

==> _eolang/paper/0BB4ABAA7A52EC9FFC0683F5B31F8337-89-phiq.tex <==
  Q.|number| ( @ -> Q.|bytes| ( @ -> [[ D> |FF-F0-00-00-00-00-00-00| ]] ) ) 

==> _eolang/paper/0E066429D0853637851228D3E7D7C38C-30-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 46 chars in the input: _eolang/paper/0E066429D0853637851228D3E7D7C38C-30-phiq.tex
% ---
% \phinoNormalize { [[ B ]] ( \tau -> e ) }{ T }
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} \phiTerminal{(} \tau \mathbin{\phiTerminal{\mapsto}} e \phiTerminal{)} }{  \phiTerminal{\bot{}} }\)\endinput

==> _eolang/paper/0E066429D0853637851228D3E7D7C38C-30-phiq.tex <==
\phinoNormalize { [[ B ]] ( \tau -> e ) }{ T }

==> _eolang/paper/0EE7A1BAB939900FD223E6223D247279-85-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 76 chars in the input: _eolang/paper/0EE7A1BAB939900FD223E6223D247279-85-phiq.tex
% ---
%   Q.|number| ( @ -> Q.|bytes| ( @ -> [[ D> |7F-F0-00-00-00-00-00-00| ]] ) ) 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{number}}{} \phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}}  \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{bytes}}{} \phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{7F-F0-00-00-00-00-00-00}}{} \phiTerminal{\rrbracket{}} \phiTerminal{)} \phiTerminal{)}\)\endinput

==> _eolang/paper/0EE7A1BAB939900FD223E6223D247279-85-phiq.tex <==
  Q.|number| ( @ -> Q.|bytes| ( @ -> [[ D> |7F-F0-00-00-00-00-00-00| ]] ) ) 

==> _eolang/paper/0FA46F946FFC9FA334F570E70F13B6E4-78-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 76 chars in the input: _eolang/paper/0FA46F946FFC9FA334F570E70F13B6E4-78-phiq.tex
% ---
%   Q.|number| ( @ -> Q.|bytes| ( @ -> [[ D> |40-09-1E-B8-51-EB-85-1F| ]] ) ) 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{number}}{} \phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}}  \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{bytes}}{} \phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{40-09-1E-B8-51-EB-85-1F}}{} \phiTerminal{\rrbracket{}} \phiTerminal{)} \phiTerminal{)}\)\endinput

==> _eolang/paper/0FA46F946FFC9FA334F570E70F13B6E4-78-phiq.tex <==
  Q.|number| ( @ -> Q.|bytes| ( @ -> [[ D> |40-09-1E-B8-51-EB-85-1F| ]] ) ) 

==> _eolang/paper/13D7EF466B6D66277145B1A1D417C0F8-16-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 8 chars in the input: _eolang/paper/13D7EF466B6D66277145B1A1D417C0F8-16-phiq.tex
% ---
% n \neq T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(n \neq  \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/13D7EF466B6D66277145B1A1D417C0F8-16-phiq.tex <==
n \neq T

==> _eolang/paper/15BAE32560A59C61D0D284D7514A21B8-15-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 44 chars in the input: _eolang/paper/15BAE32560A59C61D0D284D7514A21B8-15-phiquation.tex
% ---
% [[ |x| -> |42.0|, L> |Fn| ]] . |y| : |k|{.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{}\phiTerminal{,}\; \phiTerminal{\uplambda{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{Fn}}{} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{y}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{k}}{}{.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/15BAE32560A59C61D0D284D7514A21B8-15-phiquation.tex <==
[[ |x| -> |42.0|, L> |Fn| ]] . |y| : |k|{.}


==> _eolang/paper/17675A877415FBB3C1EC3ED3CC27B24E-10-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 40 chars in the input: _eolang/paper/17675A877415FBB3C1EC3ED3CC27B24E-10-phiq.tex
% ---
% \phinoNormalize { T ( \tau -> e ) }{ T }
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize {  \phiTerminal{\bot{}} \phiTerminal{(} \tau \mathbin{\phiTerminal{\mapsto}} e \phiTerminal{)} }{  \phiTerminal{\bot{}} }\)\endinput

==> _eolang/paper/17675A877415FBB3C1EC3ED3CC27B24E-10-phiq.tex <==
\phinoNormalize { T ( \tau -> e ) }{ T }

==> _eolang/paper/19C856855CB68088480B0F2432D9EC46-78-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 13 chars in the input: _eolang/paper/19C856855CB68088480B0F2432D9EC46-78-phiq.tex
% ---
%  b = [[ B ]] 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(b = \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/19C856855CB68088480B0F2432D9EC46-78-phiq.tex <==
 b = [[ B ]] 

==> _eolang/paper/1A5CC0A3AB1EB8C4CA5340722712A6F1-67-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 9 chars in the input: _eolang/paper/1A5CC0A3AB1EB8C4CA5340722712A6F1-67-phiq.tex
% ---
%  e:\tau  
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(e\mathord{\phiTerminal{:}}\tau\)\endinput

==> _eolang/paper/1A5CC0A3AB1EB8C4CA5340722712A6F1-67-phiq.tex <==
 e:\tau  

==> _eolang/paper/1B2A9AAC455C64DCA1C25DBFF8A97456-53-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 28 chars in the input: _eolang/paper/1B2A9AAC455C64DCA1C25DBFF8A97456-53-phiq.tex
% ---
% \phinoNormalize {b.|x|}{n_2}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize {b\phiTerminal{.}\textnormal{\texttt{x}}{}}{n_2}\)\endinput

==> _eolang/paper/1B2A9AAC455C64DCA1C25DBFF8A97456-53-phiq.tex <==
\phinoNormalize {b.|x|}{n_2}

==> _eolang/paper/1CFB045EADC3EFDF3DAEBC6C4F7FEDB0-48-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 4 chars in the input: _eolang/paper/1CFB045EADC3EFDF3DAEBC6C4F7FEDB0-48-phiq.tex
% ---
% .|y|
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{.}\textnormal{\texttt{y}}{}\)\endinput

==> _eolang/paper/1CFB045EADC3EFDF3DAEBC6C4F7FEDB0-48-phiq.tex <==
.|y|

==> _eolang/paper/1E628BCB6D55BCCB777B0DDCF9C67014-53-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 39 chars in the input: _eolang/paper/1E628BCB6D55BCCB777B0DDCF9C67014-53-phiq.tex
% ---
% \phinoDataize {n_2}{e}{s}{\delta _2}{s}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoDataize {n_2}{e}{s}{\delta _2}{s}\)\endinput

==> _eolang/paper/1E628BCB6D55BCCB777B0DDCF9C67014-53-phiq.tex <==
\phinoDataize {n_2}{e}{s}{\delta _2}{s}

==> _eolang/paper/1F1F5EA48DAE67339F8BA1716AD4DF52-117-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 21 chars in the input: _eolang/paper/1F1F5EA48DAE67339F8BA1716AD4DF52-117-phiq.tex
% ---
%  e_1 ( \tau -> e_2 ) 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(e_1 \phiTerminal{(} \tau \mathbin{\phiTerminal{\mapsto}} e_2 \phiTerminal{)}\)\endinput

==> _eolang/paper/1F1F5EA48DAE67339F8BA1716AD4DF52-117-phiq.tex <==
 e_1 ( \tau -> e_2 ) 

==> _eolang/paper/2229A3B17B0A259AC1F4802755C50C13-74-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 14 chars in the input: _eolang/paper/2229A3B17B0A259AC1F4802755C50C13-74-phiq.tex
% ---
%  \texttt {42} 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\texttt {42}\)\endinput

==> _eolang/paper/2229A3B17B0A259AC1F4802755C50C13-74-phiq.tex <==
 \texttt {42} 

==> _eolang/paper/224B72C05685D214C84A9B3C00E496BD-21-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 8 chars in the input: _eolang/paper/224B72C05685D214C84A9B3C00E496BD-21-phiq.tex
% ---
% e \neq Q
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(e \neq  \phiTerminal{\Phi{}}\)\endinput

==> _eolang/paper/224B72C05685D214C84A9B3C00E496BD-21-phiq.tex <==
e \neq Q

==> _eolang/paper/23AF4447BDA452090CDF255074B08784-123-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 14 chars in the input: _eolang/paper/23AF4447BDA452090CDF255074B08784-123-phiq.tex
% ---
% [[ |x| -> ? ]]
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}} \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/23AF4447BDA452090CDF255074B08784-123-phiq.tex <==
[[ |x| -> ? ]]

==> _eolang/paper/268C83E3CEE8611A25161A7180DE899D-19-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 37 chars in the input: _eolang/paper/268C83E3CEE8611A25161A7180DE899D-19-phiq.tex
% ---
%  \phinoContextualize { Q }{ k }{ Q } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoContextualize {  \phiTerminal{\Phi{}} }{ k }{  \phiTerminal{\Phi{}} }\)\endinput

==> _eolang/paper/268C83E3CEE8611A25161A7180DE899D-19-phiq.tex <==
 \phinoContextualize { Q }{ k }{ Q } 

==> _eolang/paper/2B55D76C86D1D49EC5ED680EE2A2E60E-15-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 49 chars in the input: _eolang/paper/2B55D76C86D1D49EC5ED680EE2A2E60E-15-phiq.tex
% ---
%  \phinoContextualize { [[ B ]] }{ k }{ [[ B ]] } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoContextualize { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} }{ k }{ \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} }\)\endinput

==> _eolang/paper/2B55D76C86D1D49EC5ED680EE2A2E60E-15-phiq.tex <==
 \phinoContextualize { [[ B ]] }{ k }{ [[ B ]] } 

==> _eolang/paper/2DFDAF211062250F90F0B98F87946117-124-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 14 chars in the input: _eolang/paper/2DFDAF211062250F90F0B98F87946117-124-phiq.tex
% ---
% [[ |x| -> b ]]
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} b \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/2DFDAF211062250F90F0B98F87946117-124-phiq.tex <==
[[ |x| -> b ]]

==> _eolang/paper/31A02BAE6F583C53FFBAF3F5AEB0FB61-43-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 58 chars in the input: _eolang/paper/31A02BAE6F583C53FFBAF3F5AEB0FB61-43-phiq.tex
% ---
%  \phinoMorph { [[ B ]] . \tau }{ e }{ s_1 }{ n_3 }{ s_3 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} \phiTerminal{.} \tau }{ e }{ s_1 }{ n_3 }{ s_3 }\)\endinput

==> _eolang/paper/31A02BAE6F583C53FFBAF3F5AEB0FB61-43-phiq.tex <==
 \phinoMorph { [[ B ]] . \tau }{ e }{ s_1 }{ n_3 }{ s_3 } 

==> _eolang/paper/345AE6A9241D0AA953F1D91C32A71E17-4-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 39 chars in the input: _eolang/paper/345AE6A9241D0AA953F1D91C32A71E17-4-phiq.tex
% ---
%  \phinoMorph { T }{ e }{ s }{ T }{ s } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph {  \phiTerminal{\bot{}} }{ e }{ s }{  \phiTerminal{\bot{}} }{ s }\)\endinput

==> _eolang/paper/345AE6A9241D0AA953F1D91C32A71E17-4-phiq.tex <==
 \phinoMorph { T }{ e }{ s }{ T }{ s } 

==> _eolang/paper/34DAE9DE6A8CDE1E1A137134859B5DE9-11-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 46 chars in the input: _eolang/paper/34DAE9DE6A8CDE1E1A137134859B5DE9-11-phiq.tex
% ---
%  \phinoNormalize { n_2 ( \tau -> k ) }{ n_3 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { n_2 \phiTerminal{(} \tau \mathbin{\phiTerminal{\mapsto}} k \phiTerminal{)} }{ n_3 }\)\endinput

==> _eolang/paper/34DAE9DE6A8CDE1E1A137134859B5DE9-11-phiq.tex <==
 \phinoNormalize { n_2 ( \tau -> k ) }{ n_3 } 

==> _eolang/paper/353F2AF0C0A0F6D1964B12AD468F4395-11-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 55 chars in the input: _eolang/paper/353F2AF0C0A0F6D1964B12AD468F4395-11-phiq.tex
% ---
%  \phinoContextualize { n_1 . \tau }{ k }{ n_2 . \tau } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoContextualize { n_1 \phiTerminal{.} \tau }{ k }{ n_2 \phiTerminal{.} \tau }\)\endinput

==> _eolang/paper/353F2AF0C0A0F6D1964B12AD468F4395-11-phiq.tex <==
 \phinoContextualize { n_1 . \tau }{ k }{ n_2 . \tau } 

==> _eolang/paper/37EBD38EC2955722BD696DBD7BED6FC1-34-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 43 chars in the input: _eolang/paper/37EBD38EC2955722BD696DBD7BED6FC1-34-phiq.tex
% ---
%  \phinoMorph { Q }{ Q }{ s_1 }{ n }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph {  \phiTerminal{\Phi{}} }{  \phiTerminal{\Phi{}} }{ s_1 }{ n }{ s_2 }\)\endinput

==> _eolang/paper/37EBD38EC2955722BD696DBD7BED6FC1-34-phiq.tex <==
 \phinoMorph { Q }{ Q }{ s_1 }{ n }{ s_2 } 

==> _eolang/paper/37F273ABC2122B7B28EC254D25A0CC7D-64-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 188 chars in the input: _eolang/paper/37F273ABC2122B7B28EC254D25A0CC7D-64-phiquation.tex
% ---
% [[ |x| -> ?, |y| -> ? ]]( |x| -> b_1 )( |y| -> b_2 ) \phiNormalize
%   \phiNormalize [[ |x| -> b_1, |y| -> ? ]] ( |y| -> b_2 ) \phiNormalize
%   \phiNormalize [[ |x| -> b_1, |y| -> b_2 ]] {.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}}\phiTerminal{,}\; \textnormal{\texttt{y}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}} \phiTerminal{\rrbracket{}}\phiTerminal{(} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} b_1 \phiTerminal{)}\phiTerminal{(} \textnormal{\texttt{y}}{} \mathbin{\phiTerminal{\mapsto}} b_2 \phiTerminal{)} \phiNormalize\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} b_1\phiTerminal{,}\; \textnormal{\texttt{y}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}} \phiTerminal{\rrbracket{}} \phiTerminal{(} \textnormal{\texttt{y}}{} \mathbin{\phiTerminal{\mapsto}} b_2 \phiTerminal{)} \phiNormalize\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} b_1\phiTerminal{,}\; \textnormal{\texttt{y}}{} \mathbin{\phiTerminal{\mapsto}} b_2 \phiTerminal{\rrbracket{}} {.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/37F273ABC2122B7B28EC254D25A0CC7D-64-phiquation.tex <==
[[ |x| -> ?, |y| -> ? ]]( |x| -> b_1 )( |y| -> b_2 ) \phiNormalize
  \phiNormalize [[ |x| -> b_1, |y| -> ? ]] ( |y| -> b_2 ) \phiNormalize
  \phiNormalize [[ |x| -> b_1, |y| -> b_2 ]] {.}


==> _eolang/paper/38D3B8BD9575DD5A26BDE53C998BB9CC-29-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 51 chars in the input: _eolang/paper/38D3B8BD9575DD5A26BDE53C998BB9CC-29-phiq.tex
% ---
%  \phinoMorph { [[ B ]] }{ e }{ s }{ [[ B ]] }{ s } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} }{ e }{ s }{ \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} }{ s }\)\endinput

==> _eolang/paper/38D3B8BD9575DD5A26BDE53C998BB9CC-29-phiq.tex <==
 \phinoMorph { [[ B ]] }{ e }{ s }{ [[ B ]] }{ s } 

==> _eolang/paper/3AAC3C27F32BF7D7AFFFAC2CCC6BDDA8-11-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 47 chars in the input: _eolang/paper/3AAC3C27F32BF7D7AFFFAC2CCC6BDDA8-11-phiq.tex
% ---
%  \phinoMorph { n_3 }{ e }{ s_2 }{ n_4 }{ s_3 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { n_3 }{ e }{ s_2 }{ n_4 }{ s_3 }\)\endinput

==> _eolang/paper/3AAC3C27F32BF7D7AFFFAC2CCC6BDDA8-11-phiq.tex <==
 \phinoMorph { n_3 }{ e }{ s_2 }{ n_4 }{ s_3 } 

==> _eolang/paper/3AAC3C27F32BF7D7AFFFAC2CCC6BDDA8-25-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 47 chars in the input: _eolang/paper/3AAC3C27F32BF7D7AFFFAC2CCC6BDDA8-25-phiq.tex
% ---
%  \phinoMorph { n_3 }{ e }{ s_2 }{ n_4 }{ s_3 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { n_3 }{ e }{ s_2 }{ n_4 }{ s_3 }\)\endinput

==> _eolang/paper/3AAC3C27F32BF7D7AFFFAC2CCC6BDDA8-25-phiq.tex <==
 \phinoMorph { n_3 }{ e }{ s_2 }{ n_4 }{ s_3 } 

==> _eolang/paper/3F8C9F9DAA9D47F1E35661E1019D9D04-33-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 52 chars in the input: _eolang/paper/3F8C9F9DAA9D47F1E35661E1019D9D04-33-phiq.tex
% ---
%  \phinoDataize { n_1 }{ e }{ s_1 }{ \delta }{ s_3 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoDataize { n_1 }{ e }{ s_1 }{ \delta }{ s_3 }\)\endinput

==> _eolang/paper/3F8C9F9DAA9D47F1E35661E1019D9D04-33-phiq.tex <==
 \phinoDataize { n_1 }{ e }{ s_1 }{ \delta }{ s_3 } 

==> _eolang/paper/3FF63787C0A4911F5CF773EF5C52F29A-123-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 10 chars in the input: _eolang/paper/3FF63787C0A4911F5CF773EF5C52F29A-123-phiq.tex
% ---
%  |x| -> b 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} b\)\endinput

==> _eolang/paper/3FF63787C0A4911F5CF773EF5C52F29A-123-phiq.tex <==
 |x| -> b 

==> _eolang/paper/40BDC089531BA40F5453FF7C0AFBCDC0-26-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 50 chars in the input: _eolang/paper/40BDC089531BA40F5453FF7C0AFBCDC0-26-phiq.tex
% ---
%  \phinoDataize { T }{ e }{ s_1 }{ \delta }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoDataize {  \phiTerminal{\bot{}} }{ e }{ s_1 }{ \delta }{ s_2 }\)\endinput

==> _eolang/paper/40BDC089531BA40F5453FF7C0AFBCDC0-26-phiq.tex <==
 \phinoDataize { T }{ e }{ s_1 }{ \delta }{ s_2 } 

==> _eolang/paper/40FAAAFE37848114A941DE5BDF3D046D-24-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 7 chars in the input: _eolang/paper/40FAAAFE37848114A941DE5BDF3D046D-24-phiq.tex
% ---
% m.\tau 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(m\phiTerminal{.}\tau\)\endinput

==> _eolang/paper/40FAAAFE37848114A941DE5BDF3D046D-24-phiq.tex <==
m.\tau 

==> _eolang/paper/419A162308495A90CB47BF6EA1BFEF0F-174-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 12 chars in the input: _eolang/paper/419A162308495A90CB47BF6EA1BFEF0F-174-phiq.tex
% ---
% Q.|x|.|next|
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{x}}{}\phiTerminal{.}\textnormal{\texttt{next}}{}\)\endinput

==> _eolang/paper/419A162308495A90CB47BF6EA1BFEF0F-174-phiq.tex <==
Q.|x|.|next|

==> _eolang/paper/43F713161F93D51B4CCC86D84C304300-28-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 90 chars in the input: _eolang/paper/43F713161F93D51B4CCC86D84C304300-28-phiquation.tex
% ---
% \label{eq:simple-application}
% [[ |x| -> ? ]]( |x| -> b ) \phiNormalize [[ |x| -> b ]] {.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation}
\begin{gathered}
\label{eq:simple-application}\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}} \phiTerminal{\rrbracket{}}\phiTerminal{(} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} b \phiTerminal{)} \phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} b \phiTerminal{\rrbracket{}} {.}
\end{gathered}
\end{equation}\endinput

==> _eolang/paper/43F713161F93D51B4CCC86D84C304300-28-phiquation.tex <==
\label{eq:simple-application}
[[ |x| -> ? ]]( |x| -> b ) \phiNormalize [[ |x| -> b ]] {.}


==> _eolang/paper/46D34CED70954CEF023A2D8682A23E91-43-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 47 chars in the input: _eolang/paper/46D34CED70954CEF023A2D8682A23E91-43-phiq.tex
% ---
%  \phinoMorph { n_2 }{ e }{ s_2 }{ n_3 }{ s_3 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { n_2 }{ e }{ s_2 }{ n_3 }{ s_3 }\)\endinput

==> _eolang/paper/46D34CED70954CEF023A2D8682A23E91-43-phiq.tex <==
 \phinoMorph { n_2 }{ e }{ s_2 }{ n_3 }{ s_3 } 

==> _eolang/paper/46D829C7B16139A1999B572C268AA6C6-45-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 48 chars in the input: _eolang/paper/46D829C7B16139A1999B572C268AA6C6-45-phiq.tex
% ---
% \phiText {if}  \tau \not = \phiTerminal {\rho } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiText {if}  \tau \not = \phiTerminal {\uprho }\)\endinput

==> _eolang/paper/46D829C7B16139A1999B572C268AA6C6-45-phiq.tex <==
\phiText {if}  \tau \not = \phiTerminal {\rho } 

==> _eolang/paper/4771DC4855EF7D3C95E606EFBEFB97A7-94-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 86 chars in the input: _eolang/paper/4771DC4855EF7D3C95E606EFBEFB97A7-94-phiquation.tex
% ---
% \label{eq:Sqrt}
% \phinoMorph{[[ L> |Sqrt|, |x| -> 256 ]]}{e}{s}{[[ D> |10-| ]]}{s} {.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation}
\begin{gathered}
\label{eq:Sqrt}\phinoMorph{\phiTerminal{\llbracket} \phiTerminal{\uplambda{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{Sqrt}}{}\phiTerminal{,}\; \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{256}}{} \phiTerminal{\rrbracket{}}}{e}{s}{\phiTerminal{\llbracket} \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{10-}}{} \phiTerminal{\rrbracket{}}}{s} {.}
\end{gathered}
\end{equation}\endinput

==> _eolang/paper/4771DC4855EF7D3C95E606EFBEFB97A7-94-phiquation.tex <==
\label{eq:Sqrt}
\phinoMorph{[[ L> |Sqrt|, |x| -> 256 ]]}{e}{s}{[[ D> |10-| ]]}{s} {.}


==> _eolang/paper/49CB6C81B38EAB083C828D95279D14ED-17-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 27 chars in the input: _eolang/paper/49CB6C81B38EAB083C828D95279D14ED-17-phiq.tex
% ---
%  \phinoNotAbsolute { n_1 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNotAbsolute { n_1 }\)\endinput

==> _eolang/paper/49CB6C81B38EAB083C828D95279D14ED-17-phiq.tex <==
 \phinoNotAbsolute { n_1 } 

==> _eolang/paper/501B970F833EFED5494D58D9B6EA3EBE-47-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 8 chars in the input: _eolang/paper/501B970F833EFED5494D58D9B6EA3EBE-47-phiq.tex
% ---
% (|t|->b)
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{(}\textnormal{\texttt{t}}{}\mathbin{\phiTerminal{\mapsto}}b\phiTerminal{)}\)\endinput

==> _eolang/paper/501B970F833EFED5494D58D9B6EA3EBE-47-phiq.tex <==
(|t|->b)

==> _eolang/paper/517BA8566FEB167AB7522972FB22778A-20-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 50 chars in the input: _eolang/paper/517BA8566FEB167AB7522972FB22778A-20-phiq.tex
% ---
%  \phinoDataize { n }{ e }{ s_2 }{ \delta }{ s_3 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoDataize { n }{ e }{ s_2 }{ \delta }{ s_3 }\)\endinput

==> _eolang/paper/517BA8566FEB167AB7522972FB22778A-20-phiq.tex <==
 \phinoDataize { n }{ e }{ s_2 }{ \delta }{ s_3 } 

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-157-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-157-phiq.tex
% ---
% @
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\upvarphi{}}\)\endinput

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-157-phiq.tex <==
@

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-158-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-158-phiq.tex
% ---
% @
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\upvarphi{}}\)\endinput

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-158-phiq.tex <==
@

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-24-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-24-phiq.tex
% ---
% @
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\upvarphi{}}\)\endinput

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-24-phiq.tex <==
@

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-26-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-26-phiq.tex
% ---
% @
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\upvarphi{}}\)\endinput

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-26-phiq.tex <==
@

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-28-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-28-phiq.tex
% ---
% @
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\upvarphi{}}\)\endinput

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-28-phiq.tex <==
@

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-30-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-30-phiq.tex
% ---
% @
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\upvarphi{}}\)\endinput

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-30-phiq.tex <==
@

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-35-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-35-phiq.tex
% ---
% @
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\upvarphi{}}\)\endinput

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-35-phiq.tex <==
@

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-44-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-44-phiq.tex
% ---
% @
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\upvarphi{}}\)\endinput

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-44-phiq.tex <==
@

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-60-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-60-phiq.tex
% ---
% @
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\upvarphi{}}\)\endinput

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-60-phiq.tex <==
@

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-69-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-69-phiq.tex
% ---
% @
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\upvarphi{}}\)\endinput

==> _eolang/paper/518ED29525738CEBDAC49C49E60EA9D3-69-phiq.tex <==
@

==> _eolang/paper/51B6C5CBFEFBE8C6F1F6877682DCDD31-12-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 72 chars in the input: _eolang/paper/51B6C5CBFEFBE8C6F1F6877682DCDD31-12-phiquation.tex
% ---
% \label{eq:price-color}
% [[ price -> ?, color -> [[ D> FF-C0-CB ]] ]] {.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation}
\begin{gathered}
\label{eq:price-color}\phiTerminal{\llbracket} \textnormal{\texttt{price}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}}\phiTerminal{,}\; \textnormal{\texttt{color}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{FF-C0-CB}}{} \phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}} {.}
\end{gathered}
\end{equation}\endinput

==> _eolang/paper/51B6C5CBFEFBE8C6F1F6877682DCDD31-12-phiquation.tex <==
\label{eq:price-color}
[[ price -> ?, color -> [[ D> FF-C0-CB ]] ]] {.}


==> _eolang/paper/5322028917BA7B637DAD6FDC02403788-28-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 31 chars in the input: _eolang/paper/5322028917BA7B637DAD6FDC02403788-28-phiq.tex
% ---
% [ D, L, @ ] \cap B = \emptyset 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\([ \phiTerminal{\Delta{}}\phiTerminal{,}\; \phiTerminal{\uplambda{}}\phiTerminal{,}\; \phiTerminal{\upvarphi{}} ] \cap B = \emptyset\)\endinput

==> _eolang/paper/5322028917BA7B637DAD6FDC02403788-28-phiq.tex <==
[ D, L, @ ] \cap B = \emptyset 

==> _eolang/paper/558EFAB3B56C4CEE40BB77A08EC5CC6A-70-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 54 chars in the input: _eolang/paper/558EFAB3B56C4CEE40BB77A08EC5CC6A-70-phiq.tex
% ---
%  \texttt {\begin {CJK}{UTF8}{gbsn}"你好"\end {CJK}} 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\texttt {\begin {CJK}{UTF8}{gbsn}\textnormal{\texttt{"你好"}}{}\end {CJK}}\)\endinput

==> _eolang/paper/558EFAB3B56C4CEE40BB77A08EC5CC6A-70-phiq.tex <==
 \texttt {\begin {CJK}{UTF8}{gbsn}"你好"\end {CJK}} 

==> _eolang/paper/5672229926CCE4C40C2114F56BE357D8-82-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 11 chars in the input: _eolang/paper/5672229926CCE4C40C2114F56BE357D8-82-phiq.tex
% ---
%   Q.|nan|  
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{nan}}{}\)\endinput

==> _eolang/paper/5672229926CCE4C40C2114F56BE357D8-82-phiq.tex <==
  Q.|nan|  

==> _eolang/paper/5B0F832AA3958C5C0A7BDCA7F6EE36D7-59-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 12 chars in the input: _eolang/paper/5B0F832AA3958C5C0A7BDCA7F6EE36D7-59-phiq.tex
% ---
%  e \not = Q 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(e \not =  \phiTerminal{\Phi{}}\)\endinput

==> _eolang/paper/5B0F832AA3958C5C0A7BDCA7F6EE36D7-59-phiq.tex <==
 e \not = Q 

==> _eolang/paper/5FE6F24D4BF1DA60E3D4F8F0B6927B67-33-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 56 chars in the input: _eolang/paper/5FE6F24D4BF1DA60E3D4F8F0B6927B67-33-phiq.tex
% ---
%  \phinoNotFormation { n_1 } \phiText {and} n_1 \not = T 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNotFormation { n_1 } \phiText {and} n_1 \not =  \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/5FE6F24D4BF1DA60E3D4F8F0B6927B67-33-phiq.tex <==
 \phinoNotFormation { n_1 } \phiText {and} n_1 \not = T 

==> _eolang/paper/605D367E222E836E0EB50848ABFE8EBB-6-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 35 chars in the input: _eolang/paper/605D367E222E836E0EB50848ABFE8EBB-6-phiquation.tex
% ---
% [[ |x| -> |k|, |k| -> |42.0| ]]{.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{k}}{}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}}{.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/605D367E222E836E0EB50848ABFE8EBB-6-phiquation.tex <==
[[ |x| -> |k|, |k| -> |42.0| ]]{.}


==> _eolang/paper/616136DDEDF69A6A308E2478D0D4B40E-20-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 52 chars in the input: _eolang/paper/616136DDEDF69A6A308E2478D0D4B40E-20-phiq.tex
% ---
%  \phinoEvaluate { [[ B ]] }{ e }{ s_1 }{ n }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoEvaluate { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} }{ e }{ s_1 }{ n }{ s_2 }\)\endinput

==> _eolang/paper/616136DDEDF69A6A308E2478D0D4B40E-20-phiq.tex <==
 \phinoEvaluate { [[ B ]] }{ e }{ s_1 }{ n }{ s_2 } 

==> _eolang/paper/6221B6179047B7FC3FD6C953AEE35581-32-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 171 chars in the input: _eolang/paper/6221B6179047B7FC3FD6C953AEE35581-32-phiquation.tex
% ---
% [[ |x| -> |t|, @ -> [[]] : |t| ]] . |x| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize [[]] : |t| : @ . |t| ( \phiTerminal{\rho} -> [[ |x| -> |t|, @ -> [[]] : |t| ]] ){.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{t}}{}\phiTerminal{,}\; \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \mathord{\phiTerminal{:}} \phiTerminal{\upvarphi{}} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{t}}{}\phiTerminal{,}\; \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{\rrbracket{}} \phiTerminal{)}{.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/6221B6179047B7FC3FD6C953AEE35581-32-phiquation.tex <==
[[ |x| -> |t|, @ -> [[]] : |t| ]] . |x| \phiNormalize[\nameref{r:dot}]
  \phiNormalize [[]] : |t| : @ . |t| ( \phiTerminal{\rho} -> [[ |x| -> |t|, @ -> [[]] : |t| ]] ){.}


==> _eolang/paper/628FFAB53DA4CE925A5086C57422198B-8-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 257 chars in the input: _eolang/paper/628FFAB53DA4CE925A5086C57422198B-8-phiquation.tex
% ---
% \label{eq:celsius}
% [[
%   @ -> [[ @ -> |c| . |times| ( |x| -> |1.8| ) . |plus| ( |x| -> |32.0| ), |c| -> |25.0| ]],
%   |bytes|(@) -> [[]],
%   |number|(@) -> [[ |times|(|x|, \phiTerminal{\rho}) -> |Fn1| : L, |plus|(|x|, \phiTerminal{\rho}) -> |Fn2| : L ]]
% ]]{.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation}
\begin{split}
&\label{eq:celsius}\phiTerminal{\llbracket}\phiEOL{}
& \quad{}\phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{c}}{} \phiTerminal{.} \textnormal{\texttt{times}}{} \phiTerminal{(} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{1.8}}{} \phiTerminal{)} \phiTerminal{.} \textnormal{\texttt{plus}}{} \phiTerminal{(} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{32.0}}{} \phiTerminal{)}\phiTerminal{,}\; \textnormal{\texttt{c}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{25.0}}{} \phiTerminal{\rrbracket{}}\phiTerminal{,}\;\phiEOL{}
& \quad{}\textnormal{\texttt{bytes}}{}\phiTerminal{(}\phiTerminal{\upvarphi{}}\phiTerminal{)} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}}\phiTerminal{,}\;\phiEOL{}
& \quad{}\textnormal{\texttt{number}}{}\phiTerminal{(}\phiTerminal{\upvarphi{}}\phiTerminal{)} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \textnormal{\texttt{times}}{}\phiTerminal{(}\textnormal{\texttt{x}}{}\phiTerminal{,}\; \phiTerminal{\uprho}\phiTerminal{)} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{Fn1}}{} \mathord{\phiTerminal{:}} \phiTerminal{\uplambda{}}\phiTerminal{,}\; \textnormal{\texttt{plus}}{}\phiTerminal{(}\textnormal{\texttt{x}}{}\phiTerminal{,}\; \phiTerminal{\uprho}\phiTerminal{)} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{Fn2}}{} \mathord{\phiTerminal{:}} \phiTerminal{\uplambda{}} \phiTerminal{\rrbracket{}}\phiEOL{}
&\phiTerminal{\rrbracket{}}{.}
\end{split}
\end{equation}\endinput

==> _eolang/paper/628FFAB53DA4CE925A5086C57422198B-8-phiquation.tex <==
\label{eq:celsius}
[[
  @ -> [[ @ -> |c| . |times| ( |x| -> |1.8| ) . |plus| ( |x| -> |32.0| ), |c| -> |25.0| ]],
  |bytes|(@) -> [[]],
  |number|(@) -> [[ |times|(|x|, \phiTerminal{\rho}) -> |Fn1| : L, |plus|(|x|, \phiTerminal{\rho}) -> |Fn2| : L ]]
]]{.}


==> _eolang/paper/638A4051EAD127D0CE4CD8073B28D2EA-64-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 20 chars in the input: _eolang/paper/638A4051EAD127D0CE4CD8073B28D2EA-64-phiq.tex
% ---
%  \tau _1 -> \tau _2 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\tau _1 \mathbin{\phiTerminal{\mapsto}} \tau _2\)\endinput

==> _eolang/paper/638A4051EAD127D0CE4CD8073B28D2EA-64-phiq.tex <==
 \tau _1 -> \tau _2 

==> _eolang/paper/641300E2ADC0ED981424D37C4DE593BD-26-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 56 chars in the input: _eolang/paper/641300E2ADC0ED981424D37C4DE593BD-26-phiq.tex
% ---
%  \phinoDataize { [[ B ]] }{ e }{ s_1 }{ \delta }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoDataize { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} }{ e }{ s_1 }{ \delta }{ s_2 }\)\endinput

==> _eolang/paper/641300E2ADC0ED981424D37C4DE593BD-26-phiq.tex <==
 \phinoDataize { [[ B ]] }{ e }{ s_1 }{ \delta }{ s_2 } 

==> _eolang/paper/641300E2ADC0ED981424D37C4DE593BD-7-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 56 chars in the input: _eolang/paper/641300E2ADC0ED981424D37C4DE593BD-7-phiq.tex
% ---
%  \phinoDataize { [[ B ]] }{ e }{ s_1 }{ \delta }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoDataize { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} }{ e }{ s_1 }{ \delta }{ s_2 }\)\endinput

==> _eolang/paper/641300E2ADC0ED981424D37C4DE593BD-7-phiq.tex <==
 \phinoDataize { [[ B ]] }{ e }{ s_1 }{ \delta }{ s_2 } 

==> _eolang/paper/648EF51DAA60E3B453FD0B8BBE13EE9A-33-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 52 chars in the input: _eolang/paper/648EF51DAA60E3B453FD0B8BBE13EE9A-33-phiq.tex
% ---
%  \phinoDataize { n_2 }{ e }{ s_2 }{ \delta }{ s_3 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoDataize { n_2 }{ e }{ s_2 }{ \delta }{ s_3 }\)\endinput

==> _eolang/paper/648EF51DAA60E3B453FD0B8BBE13EE9A-33-phiq.tex <==
 \phinoDataize { n_2 }{ e }{ s_2 }{ \delta }{ s_3 } 

==> _eolang/paper/6560AE1213A4CD1AA5E71C459C857F28-67-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1006 chars in the input: _eolang/paper/6560AE1213A4CD1AA5E71C459C857F28-67-phiquation.tex
% ---
% \phinoMeet{basic-l:1}{ [[ |x| -> ? : |t| ( |t| -> |k| ), |k| -> |Fn| : L ]] } . |x| . |t| . |p| : |a| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize ? : |t| ( |t| -> |Fn| : L : |k| . |k|, \phiTerminal{\rho} -> \phinoAgain{basic-l:1} ) . |t| . |p| : |a| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize ? : |t| ( |t| -> |Fn| : L ( \phiTerminal{\rho} -> |Fn| : L : |k| ), \phiTerminal{\rho} -> \phinoAgain{basic-l:1} ) . |t| . |p| : |a| \phiNormalize[\nameref{r:skip}]
%   \phiNormalize ? : |t| ( |t| -> |Fn| : L, \phiTerminal{\rho} -> \phinoAgain{basic-l:1} ) . |t| . |p| : |a| \phiNormalize[\nameref{r:copy}]
%   \phiNormalize \phinoMeet{basic-l:2}{ |Fn| : L : |t| } ( \phiTerminal{\rho} -> \phinoAgain{basic-l:1} ) . |t| . |p| : |a| \phiNormalize[\nameref{r:skip}]
%   \phiNormalize \phinoAgain{basic-l:2} . |t| . |p| : |a| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize |Fn| : L ( \phiTerminal{\rho} -> \phinoAgain{basic-l:2} ) . |p| : |a| \phiNormalize[\nameref{r:skip}]
%   \phiNormalize |Fn| : L . |p| : |a|{.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phinoMeet{basic-l:1}{ \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{(} \textnormal{\texttt{t}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{k}}{} \phiTerminal{)}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{Fn}}{} \mathord{\phiTerminal{:}} \phiTerminal{\uplambda{}} \phiTerminal{\rrbracket{}} } \phiTerminal{.} \textnormal{\texttt{x}}{} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{.} \textnormal{\texttt{p}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{a}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\varnothing{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{(} \textnormal{\texttt{t}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{Fn}}{} \mathord{\phiTerminal{:}} \phiTerminal{\uplambda{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{k}}{} \phiTerminal{.} \textnormal{\texttt{k}}{}\phiTerminal{,}\; \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-l:1} \phiTerminal{)} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{.} \textnormal{\texttt{p}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{a}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\varnothing{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{(} \textnormal{\texttt{t}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{Fn}}{} \mathord{\phiTerminal{:}} \phiTerminal{\uplambda{}} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{Fn}}{} \mathord{\phiTerminal{:}} \phiTerminal{\uplambda{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{k}}{} \phiTerminal{)}\phiTerminal{,}\; \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-l:1} \phiTerminal{)} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{.} \textnormal{\texttt{p}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{a}}{} \phiNormalize[\nameref{r:skip}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\varnothing{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{(} \textnormal{\texttt{t}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{Fn}}{} \mathord{\phiTerminal{:}} \phiTerminal{\uplambda{}}\phiTerminal{,}\; \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-l:1} \phiTerminal{)} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{.} \textnormal{\texttt{p}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{a}}{} \phiNormalize[\nameref{r:copy}]\phiEOL{}
& \quad{}\phiNormalize \phinoMeet{basic-l:2}{ \textnormal{\texttt{Fn}}{} \mathord{\phiTerminal{:}} \phiTerminal{\uplambda{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} } \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-l:1} \phiTerminal{)} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{.} \textnormal{\texttt{p}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{a}}{} \phiNormalize[\nameref{r:skip}]\phiEOL{}
& \quad{}\phiNormalize \phinoAgain{basic-l:2} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{.} \textnormal{\texttt{p}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{a}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \textnormal{\texttt{Fn}}{} \mathord{\phiTerminal{:}} \phiTerminal{\uplambda{}} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-l:2} \phiTerminal{)} \phiTerminal{.} \textnormal{\texttt{p}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{a}}{} \phiNormalize[\nameref{r:skip}]\phiEOL{}
& \quad{}\phiNormalize \textnormal{\texttt{Fn}}{} \mathord{\phiTerminal{:}} \phiTerminal{\uplambda{}} \phiTerminal{.} \textnormal{\texttt{p}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{a}}{}{.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/6560AE1213A4CD1AA5E71C459C857F28-67-phiquation.tex <==
\phinoMeet{basic-l:1}{ [[ |x| -> ? : |t| ( |t| -> |k| ), |k| -> |Fn| : L ]] } . |x| . |t| . |p| : |a| \phiNormalize[\nameref{r:dot}]
  \phiNormalize ? : |t| ( |t| -> |Fn| : L : |k| . |k|, \phiTerminal{\rho} -> \phinoAgain{basic-l:1} ) . |t| . |p| : |a| \phiNormalize[\nameref{r:dot}]
  \phiNormalize ? : |t| ( |t| -> |Fn| : L ( \phiTerminal{\rho} -> |Fn| : L : |k| ), \phiTerminal{\rho} -> \phinoAgain{basic-l:1} ) . |t| . |p| : |a| \phiNormalize[\nameref{r:skip}]
  \phiNormalize ? : |t| ( |t| -> |Fn| : L, \phiTerminal{\rho} -> \phinoAgain{basic-l:1} ) . |t| . |p| : |a| \phiNormalize[\nameref{r:copy}]
  \phiNormalize \phinoMeet{basic-l:2}{ |Fn| : L : |t| } ( \phiTerminal{\rho} -> \phinoAgain{basic-l:1} ) . |t| . |p| : |a| \phiNormalize[\nameref{r:skip}]
  \phiNormalize \phinoAgain{basic-l:2} . |t| . |p| : |a| \phiNormalize[\nameref{r:dot}]
  \phiNormalize |Fn| : L ( \phiTerminal{\rho} -> \phinoAgain{basic-l:2} ) . |p| : |a| \phiNormalize[\nameref{r:skip}]
  \phiNormalize |Fn| : L . |p| : |a|{.}


==> _eolang/paper/6BF3226421EC5088618D64B737C43E2A-177-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 16 chars in the input: _eolang/paper/6BF3226421EC5088618D64B737C43E2A-177-phiq.tex
% ---
%  Q.|k|.|next|.^ 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{k}}{}\phiTerminal{.}\textnormal{\texttt{next}}{}\phiTerminal{.}\phiTerminal{\uprho{}}\)\endinput

==> _eolang/paper/6BF3226421EC5088618D64B737C43E2A-177-phiq.tex <==
 Q.|k|.|next|.^ 

==> _eolang/paper/6DDB3FCE2A7AA3A30F246C0853DFBC6F-35-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 55 chars in the input: _eolang/paper/6DDB3FCE2A7AA3A30F246C0853DFBC6F-35-phiq.tex
% ---
% \phinoNormalize { [[ B ]] . \phiTerminal {\rho } }{ T }
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} \phiTerminal{.} \phiTerminal {\uprho } }{  \phiTerminal{\bot{}} }\)\endinput

==> _eolang/paper/6DDB3FCE2A7AA3A30F246C0853DFBC6F-35-phiq.tex <==
\phinoNormalize { [[ B ]] . \phiTerminal {\rho } }{ T }

==> _eolang/paper/720D769440BD4A151FDF40581FF9BCE7-25-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 78 chars in the input: _eolang/paper/720D769440BD4A151FDF40581FF9BCE7-25-phiq.tex
% ---
% \phiText {if}  [ D \char 44{} L ] \not \subseteq \lparen B_1 \cup B_2 \rparen 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiText {if}  [ \phiTerminal{\Delta{}} \char 44{} \phiTerminal{\uplambda{}} ] \not \subseteq \lparen B_1 \cup B_2 \rparen\)\endinput

==> _eolang/paper/720D769440BD4A151FDF40581FF9BCE7-25-phiq.tex <==
\phiText {if}  [ D \char 44{} L ] \not \subseteq \lparen B_1 \cup B_2 \rparen 

==> _eolang/paper/741BA85BDA6FE6D2B45A0132822CC859-25-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 54 chars in the input: _eolang/paper/741BA85BDA6FE6D2B45A0132822CC859-25-phiq.tex
% ---
%  \phinoMorph { n_1 . \tau }{ e }{ s_1 }{ n_4 }{ s_3 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { n_1 \phiTerminal{.} \tau }{ e }{ s_1 }{ n_4 }{ s_3 }\)\endinput

==> _eolang/paper/741BA85BDA6FE6D2B45A0132822CC859-25-phiq.tex <==
 \phinoMorph { n_1 . \tau }{ e }{ s_1 }{ n_4 }{ s_3 } 

==> _eolang/paper/7532C8DAF9D7B1E252E41EA46ABD48BA-51-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 65 chars in the input: _eolang/paper/7532C8DAF9D7B1E252E41EA46ABD48BA-51-phiq.tex
% ---
%  @ \in B \phiText {and} [ \tau \char 44{} L ] \cap B = \emptyset 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\upvarphi{}} \in B \phiText {and} [ \tau \char 44{} \phiTerminal{\uplambda{}} ] \cap B = \emptyset\)\endinput

==> _eolang/paper/7532C8DAF9D7B1E252E41EA46ABD48BA-51-phiq.tex <==
 @ \in B \phiText {and} [ \tau \char 44{} L ] \cap B = \emptyset 

==> _eolang/paper/770A80DDD18F4EEEF7637C7B41C61836-141-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 10 chars in the input: _eolang/paper/770A80DDD18F4EEEF7637C7B41C61836-141-phiq.tex
% ---
%  e . \tau 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(e \phiTerminal{.} \tau\)\endinput

==> _eolang/paper/770A80DDD18F4EEEF7637C7B41C61836-141-phiq.tex <==
 e . \tau 

==> _eolang/paper/77383D586A78508878922960E5BCB0D3-17-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 61 chars in the input: _eolang/paper/77383D586A78508878922960E5BCB0D3-17-phiq.tex
% ---
%  \phinoMorph { n ( \tau -> n_1 ) }{ e }{ s_1 }{ n_2 }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { n \phiTerminal{(} \tau \mathbin{\phiTerminal{\mapsto}} n_1 \phiTerminal{)} }{ e }{ s_1 }{ n_2 }{ s_2 }\)\endinput

==> _eolang/paper/77383D586A78508878922960E5BCB0D3-17-phiq.tex <==
 \phinoMorph { n ( \tau -> n_1 ) }{ e }{ s_1 }{ n_2 }{ s_2 } 

==> _eolang/paper/795957AC07A8B06652757BBC0A1B36B6-102-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 62 chars in the input: _eolang/paper/795957AC07A8B06652757BBC0A1B36B6-102-phiquation.tex
% ---
% \phinoDataize{[[ L> |Sqrt|, |x| -> 256 ]]}{e}{s}{|16|}{s} {.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
\phinoDataize{\phiTerminal{\llbracket} \phiTerminal{\uplambda{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{Sqrt}}{}\phiTerminal{,}\; \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{256}}{} \phiTerminal{\rrbracket{}}}{e}{s}{\textnormal{\texttt{16}}{}}{s} {.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/795957AC07A8B06652757BBC0A1B36B6-102-phiquation.tex <==
\phinoDataize{[[ L> |Sqrt|, |x| -> 256 ]]}{e}{s}{|16|}{s} {.}


==> _eolang/paper/7A19ED7FC71D456241C084606A156492-11-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 47 chars in the input: _eolang/paper/7A19ED7FC71D456241C084606A156492-11-phiq.tex
% ---
%  \phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 }\)\endinput

==> _eolang/paper/7A19ED7FC71D456241C084606A156492-11-phiq.tex <==
 \phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 } 

==> _eolang/paper/7A19ED7FC71D456241C084606A156492-25-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 47 chars in the input: _eolang/paper/7A19ED7FC71D456241C084606A156492-25-phiq.tex
% ---
%  \phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 }\)\endinput

==> _eolang/paper/7A19ED7FC71D456241C084606A156492-25-phiq.tex <==
 \phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 } 

==> _eolang/paper/7A19ED7FC71D456241C084606A156492-33-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 47 chars in the input: _eolang/paper/7A19ED7FC71D456241C084606A156492-33-phiq.tex
% ---
%  \phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 }\)\endinput

==> _eolang/paper/7A19ED7FC71D456241C084606A156492-33-phiq.tex <==
 \phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 } 

==> _eolang/paper/7A19ED7FC71D456241C084606A156492-51-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 47 chars in the input: _eolang/paper/7A19ED7FC71D456241C084606A156492-51-phiq.tex
% ---
%  \phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 }\)\endinput

==> _eolang/paper/7A19ED7FC71D456241C084606A156492-51-phiq.tex <==
 \phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 } 

==> _eolang/paper/7A19ED7FC71D456241C084606A156492-59-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 47 chars in the input: _eolang/paper/7A19ED7FC71D456241C084606A156492-59-phiq.tex
% ---
%  \phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 }\)\endinput

==> _eolang/paper/7A19ED7FC71D456241C084606A156492-59-phiq.tex <==
 \phinoMorph { n_1 }{ e }{ s_1 }{ n_2 }{ s_2 } 

==> _eolang/paper/7A7E7F00473D8B29D78EA4AD83339A3F-46-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 4 chars in the input: _eolang/paper/7A7E7F00473D8B29D78EA4AD83339A3F-46-phiq.tex
% ---
% .|p|
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{.}\textnormal{\texttt{p}}{}\)\endinput

==> _eolang/paper/7A7E7F00473D8B29D78EA4AD83339A3F-46-phiq.tex <==
.|p|

==> _eolang/paper/7E6A2AFE551E067A75FAFACF47A6D981-162-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/7E6A2AFE551E067A75FAFACF47A6D981-162-phiq.tex
% ---
% ^
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uprho{}}\)\endinput

==> _eolang/paper/7E6A2AFE551E067A75FAFACF47A6D981-162-phiq.tex <==
^

==> _eolang/paper/7E6A2AFE551E067A75FAFACF47A6D981-28-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/7E6A2AFE551E067A75FAFACF47A6D981-28-phiq.tex
% ---
% ^
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uprho{}}\)\endinput

==> _eolang/paper/7E6A2AFE551E067A75FAFACF47A6D981-28-phiq.tex <==
^

==> _eolang/paper/7E6A2AFE551E067A75FAFACF47A6D981-36-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/7E6A2AFE551E067A75FAFACF47A6D981-36-phiq.tex
% ---
% ^
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uprho{}}\)\endinput

==> _eolang/paper/7E6A2AFE551E067A75FAFACF47A6D981-36-phiq.tex <==
^

==> _eolang/paper/7E89B0EEFBC31D6453377B2AD3BBF3F3-27-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 55 chars in the input: _eolang/paper/7E89B0EEFBC31D6453377B2AD3BBF3F3-27-phiq.tex
% ---
%  \phinoContextualize { \phiTerminal {\xi } }{ k }{ k } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoContextualize { \phiTerminal {\upxi } }{ k }{ k }\)\endinput

==> _eolang/paper/7E89B0EEFBC31D6453377B2AD3BBF3F3-27-phiq.tex <==
 \phinoContextualize { \phiTerminal {\xi } }{ k }{ k } 

==> _eolang/paper/808163C8AF5A656D71B7841A47959225-25-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 130 chars in the input: _eolang/paper/808163C8AF5A656D71B7841A47959225-25-phiq.tex
% ---
% \phiText {if}  \phinoContextualize { n }{ [[ B_1, B_2 ]] }{ e_1 } \phiText {and} \phinoNamed { e_2 }{ [[ B_1, \tau -> n, B_2 ]] } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiText {if}  \phinoContextualize { n }{ \phiTerminal{\llbracket} B_1\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} }{ e_1 } \phiText {and} \phinoNamed { e_2 }{ \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \tau \mathbin{\phiTerminal{\mapsto}} n\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} }\)\endinput

==> _eolang/paper/808163C8AF5A656D71B7841A47959225-25-phiq.tex <==
\phiText {if}  \phinoContextualize { n }{ [[ B_1, B_2 ]] }{ e_1 } \phiText {and} \phinoNamed { e_2 }{ [[ B_1, \tau -> n, B_2 ]] } 

==> _eolang/paper/8487DE8AFE0AAA22153E188203FC850D-59-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 45 chars in the input: _eolang/paper/8487DE8AFE0AAA22153E188203FC850D-59-phiq.tex
% ---
%  \phinoMorph { Q }{ e }{ s_1 }{ n_2 }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph {  \phiTerminal{\Phi{}} }{ e }{ s_1 }{ n_2 }{ s_2 }\)\endinput

==> _eolang/paper/8487DE8AFE0AAA22153E188203FC850D-59-phiq.tex <==
 \phinoMorph { Q }{ e }{ s_1 }{ n_2 }{ s_2 } 

==> _eolang/paper/88628EEC756046DB15B496B0EB94E4E1-25-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 39 chars in the input: _eolang/paper/88628EEC756046DB15B496B0EB94E4E1-25-phiq.tex
% ---
%  \phinoNormalize { n_2 . \tau }{ n_3 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { n_2 \phiTerminal{.} \tau }{ n_3 }\)\endinput

==> _eolang/paper/88628EEC756046DB15B496B0EB94E4E1-25-phiq.tex <==
 \phinoNormalize { n_2 . \tau }{ n_3 } 

==> _eolang/paper/886E07BE4A11F3A4D05050AF170A3047-155-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 89 chars in the input: _eolang/paper/886E07BE4A11F3A4D05050AF170A3047-155-phiq.tex
% ---
%  \langle e_1 {,}\; s_2 \rangle = f \lparen [[ B_1, L>f, B_2 ]] {,}\; e {,}\; s_1 \rparen 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\langle e_1 {,}\; s_2 \rangle = f \lparen \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \phiTerminal{\uplambda{}} \mathbin{\phiTerminal{\phiDotted}}f\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} {,}\; e {,}\; s_1 \rparen\)\endinput

==> _eolang/paper/886E07BE4A11F3A4D05050AF170A3047-155-phiq.tex <==
 \langle e_1 {,}\; s_2 \rangle = f \lparen [[ B_1, L>f, B_2 ]] {,}\; e {,}\; s_1 \rparen 

==> _eolang/paper/89FD566E988E79B01B4AAAB11A608376-28-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 128 chars in the input: _eolang/paper/89FD566E988E79B01B4AAAB11A608376-28-phiquation.tex
% ---
% [[ |x| -> |t|, |t| -> ? ]] ( |t| -> |42.0| ) \phiNormalize[\nameref{r:copy}]
%   \phiNormalize [[ |x| -> |t|, |t| -> |42.0| ]]{.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{t}}{}\phiTerminal{,}\; \textnormal{\texttt{t}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}} \phiTerminal{\rrbracket{}} \phiTerminal{(} \textnormal{\texttt{t}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{)} \phiNormalize[\nameref{r:copy}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{t}}{}\phiTerminal{,}\; \textnormal{\texttt{t}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}}{.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/89FD566E988E79B01B4AAAB11A608376-28-phiquation.tex <==
[[ |x| -> |t|, |t| -> ? ]] ( |t| -> |42.0| ) \phiNormalize[\nameref{r:copy}]
  \phiNormalize [[ |x| -> |t|, |t| -> |42.0| ]]{.}


==> _eolang/paper/8B869221DB1F5B1114BE2B1BA655376A-6-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 71 chars in the input: _eolang/paper/8B869221DB1F5B1114BE2B1BA655376A-6-phiq.tex
% ---
%  \phinoContextualize { n_1 ( \tau -> e ) }{ k }{ n_2 ( \tau -> n_3 ) } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoContextualize { n_1 \phiTerminal{(} \tau \mathbin{\phiTerminal{\mapsto}} e \phiTerminal{)} }{ k }{ n_2 \phiTerminal{(} \tau \mathbin{\phiTerminal{\mapsto}} n_3 \phiTerminal{)} }\)\endinput

==> _eolang/paper/8B869221DB1F5B1114BE2B1BA655376A-6-phiq.tex <==
 \phinoContextualize { n_1 ( \tau -> e ) }{ k }{ n_2 ( \tau -> n_3 ) } 

==> _eolang/paper/8F5387022669D0C5F3904E1C321DA05F-78-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 50 chars in the input: _eolang/paper/8F5387022669D0C5F3904E1C321DA05F-78-phiquation.tex
% ---
% [[ @ -> [[ |x| -> b ]] ]].|x| \phiNormalize b {.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
\phiTerminal{\llbracket} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} b \phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}}\phiTerminal{.}\textnormal{\texttt{x}}{} \phiNormalize b {.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/8F5387022669D0C5F3904E1C321DA05F-78-phiquation.tex <==
[[ @ -> [[ |x| -> b ]] ]].|x| \phiNormalize b {.}


==> _eolang/paper/8F8A31A98332A9EB07A6B320790F8950-74-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 76 chars in the input: _eolang/paper/8F8A31A98332A9EB07A6B320790F8950-74-phiq.tex
% ---
%   Q.|number| ( @ -> Q.|bytes| ( @ -> [[ D> |40-45-00-00-00-00-00-00| ]] ) ) 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{number}}{} \phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}}  \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{bytes}}{} \phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{40-45-00-00-00-00-00-00}}{} \phiTerminal{\rrbracket{}} \phiTerminal{)} \phiTerminal{)}\)\endinput

==> _eolang/paper/8F8A31A98332A9EB07A6B320790F8950-74-phiq.tex <==
  Q.|number| ( @ -> Q.|bytes| ( @ -> [[ D> |40-45-00-00-00-00-00-00| ]] ) ) 

==> _eolang/paper/9123F88D0A5D96D30AE707560ED29ADB-40-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 610 chars in the input: _eolang/paper/9123F88D0A5D96D30AE707560ED29ADB-40-phiquation.tex
% ---
% \phinoMeet{basic-i:1}{ \phiTerminal{\rho} . \phiTerminal{\rho} . |t| : |x| } . |x| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize [[]] . \phiTerminal{\rho} . \phiTerminal{\rho} . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-i:1} ) \phiNormalize[\nameref{r:norho}]
%   \phiNormalize T . \phiTerminal{\rho} . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-i:1} ) \phiNormalize[\nameref{r:dd}]
%   \phiNormalize T . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-i:1} ) \phiNormalize[\nameref{r:dd}]
%   \phiNormalize T ( \phiTerminal{\rho} -> \phinoAgain{basic-i:1} ) \phiNormalize[\nameref{r:dc}]
%   \phiNormalize T{.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phinoMeet{basic-i:1}{ \phiTerminal{\uprho} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{t}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{x}}{} } \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-i:1} \phiTerminal{)} \phiNormalize[\nameref{r:norho}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-i:1} \phiTerminal{)} \phiNormalize[\nameref{r:dd}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-i:1} \phiTerminal{)} \phiNormalize[\nameref{r:dd}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-i:1} \phiTerminal{)} \phiNormalize[\nameref{r:dc}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}}{.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/9123F88D0A5D96D30AE707560ED29ADB-40-phiquation.tex <==
\phinoMeet{basic-i:1}{ \phiTerminal{\rho} . \phiTerminal{\rho} . |t| : |x| } . |x| \phiNormalize[\nameref{r:dot}]
  \phiNormalize [[]] . \phiTerminal{\rho} . \phiTerminal{\rho} . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-i:1} ) \phiNormalize[\nameref{r:norho}]
  \phiNormalize T . \phiTerminal{\rho} . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-i:1} ) \phiNormalize[\nameref{r:dd}]
  \phiNormalize T . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-i:1} ) \phiNormalize[\nameref{r:dd}]
  \phiNormalize T ( \phiTerminal{\rho} -> \phinoAgain{basic-i:1} ) \phiNormalize[\nameref{r:dc}]
  \phiNormalize T{.}


==> _eolang/paper/924D738C76E2F2150AF9E02C25EB385F-3-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 26 chars in the input: _eolang/paper/924D738C76E2F2150AF9E02C25EB385F-3-phiquation.tex
% ---
% ? : |x| ( |x| -> |t| ){.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
\phiTerminal{\varnothing{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{x}}{} \phiTerminal{(} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{t}}{} \phiTerminal{)}{.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/924D738C76E2F2150AF9E02C25EB385F-3-phiquation.tex <==
? : |x| ( |x| -> |t| ){.}


==> _eolang/paper/965B4FD5D37B074E328CBDC86F1928BC-20-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 49 chars in the input: _eolang/paper/965B4FD5D37B074E328CBDC86F1928BC-20-phiq.tex
% ---
%  L \in B \phiText {and} [ D ] \cap B = \emptyset 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}} \in B \phiText {and} [ \phiTerminal{\Delta{}} ] \cap B = \emptyset\)\endinput

==> _eolang/paper/965B4FD5D37B074E328CBDC86F1928BC-20-phiq.tex <==
 L \in B \phiText {and} [ D ] \cap B = \emptyset 

==> _eolang/paper/97E7794F66FF14DC39EBDEFAA1ED0075-172-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 106 chars in the input: _eolang/paper/97E7794F66FF14DC39EBDEFAA1ED0075-172-phiquation.tex
% ---
% [[ |x| -> [[ |a| -> ?, next -> [[ @ -> $.^.|a|.plus( |x| -> 1 ) ]] ]], |k| -> $.|x|( |a| -> |42| ) ]] {.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \textnormal{\texttt{a}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}}\phiTerminal{,}\; \textnormal{\texttt{next}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\upxi{}}\phiTerminal{.}\phiTerminal{\uprho{}}\phiTerminal{.}\textnormal{\texttt{a}}{}\phiTerminal{.}\textnormal{\texttt{plus}}{}\phiTerminal{(} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{1}}{} \phiTerminal{)} \phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\upxi{}}\phiTerminal{.}\textnormal{\texttt{x}}{}\phiTerminal{(} \textnormal{\texttt{a}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42}}{} \phiTerminal{)} \phiTerminal{\rrbracket{}} {.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/97E7794F66FF14DC39EBDEFAA1ED0075-172-phiquation.tex <==
[[ |x| -> [[ |a| -> ?, next -> [[ @ -> $.^.|a|.plus( |x| -> 1 ) ]] ]], |k| -> $.|x|( |a| -> |42| ) ]] {.}


==> _eolang/paper/993DB34C574F72463144C9C9E304AE36-89-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 12 chars in the input: _eolang/paper/993DB34C574F72463144C9C9E304AE36-89-phiq.tex
% ---
%   Q.|ninf|  
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{ninf}}{}\)\endinput

==> _eolang/paper/993DB34C574F72463144C9C9E304AE36-89-phiq.tex <==
  Q.|ninf|  

==> _eolang/paper/9B55DA972C1E593F6328AF176BEB2BE8-53-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 39 chars in the input: _eolang/paper/9B55DA972C1E593F6328AF176BEB2BE8-53-phiq.tex
% ---
% \phinoDataize {n_1}{e}{s}{\delta _1}{s}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoDataize {n_1}{e}{s}{\delta _1}{s}\)\endinput

==> _eolang/paper/9B55DA972C1E593F6328AF176BEB2BE8-53-phiq.tex <==
\phinoDataize {n_1}{e}{s}{\delta _1}{s}

==> _eolang/paper/9B8CA31992E2CA1C57855AA160B0920C-34-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 43 chars in the input: _eolang/paper/9B8CA31992E2CA1C57855AA160B0920C-34-phiq.tex
% ---
%  \phinoMorph { T }{ Q }{ s_1 }{ n }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph {  \phiTerminal{\bot{}} }{  \phiTerminal{\Phi{}} }{ s_1 }{ n }{ s_2 }\)\endinput

==> _eolang/paper/9B8CA31992E2CA1C57855AA160B0920C-34-phiq.tex <==
 \phinoMorph { T }{ Q }{ s_1 }{ n }{ s_2 } 

==> _eolang/paper/9C9047B0EA1AAEB7CEB797C8BA6DC532-43-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 128 chars in the input: _eolang/paper/9C9047B0EA1AAEB7CEB797C8BA6DC532-43-phiquation.tex
% ---
% \label{eq:dot-notation}
% [[ |x| -> \phiOver{$.|p|(|t| -> b)}.|y|, |p| -> [[ |t| -> ?, |y| -> $.|t| ]] ]].|x| \phiNormalize b {.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation}
\begin{gathered}
\label{eq:dot-notation}\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiOver{\phiTerminal{\upxi{}}\phiTerminal{.}\textnormal{\texttt{p}}{}\phiTerminal{(}\textnormal{\texttt{t}}{} \mathbin{\phiTerminal{\mapsto}} b\phiTerminal{)}}\phiTerminal{.}\textnormal{\texttt{y}}{}\phiTerminal{,}\; \textnormal{\texttt{p}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \textnormal{\texttt{t}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}}\phiTerminal{,}\; \textnormal{\texttt{y}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\upxi{}}\phiTerminal{.}\textnormal{\texttt{t}}{} \phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}}\phiTerminal{.}\textnormal{\texttt{x}}{} \phiNormalize b {.}
\end{gathered}
\end{equation}\endinput

==> _eolang/paper/9C9047B0EA1AAEB7CEB797C8BA6DC532-43-phiquation.tex <==
\label{eq:dot-notation}
[[ |x| -> \phiOver{$.|p|(|t| -> b)}.|y|, |p| -> [[ |t| -> ?, |y| -> $.|t| ]] ]].|x| \phiNormalize b {.}


==> _eolang/paper/9D1C886CD8F04691D880144BB0ABCD7F-25-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 28 chars in the input: _eolang/paper/9D1C886CD8F04691D880144BB0ABCD7F-25-phiq.tex
% ---
%  \phinoNotFormation { n_1 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNotFormation { n_1 }\)\endinput

==> _eolang/paper/9D1C886CD8F04691D880144BB0ABCD7F-25-phiq.tex <==
 \phinoNotFormation { n_1 } 

==> _eolang/paper/9E08F8285C57929DD89FFD5EEBB0FB51-53-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 30 chars in the input: _eolang/paper/9E08F8285C57929DD89FFD5EEBB0FB51-53-phiq.tex
% ---
% \delta = \delta _1 + \delta _2
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\delta = \delta _1 + \delta _2\)\endinput

==> _eolang/paper/9E08F8285C57929DD89FFD5EEBB0FB51-53-phiq.tex <==
\delta = \delta _1 + \delta _2

==> _eolang/paper/9FBFA353E4EA74C38ACA4A758EB912D4-58-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 47 chars in the input: _eolang/paper/9FBFA353E4EA74C38ACA4A758EB912D4-58-phiq.tex
% ---
%  e ( \tau _1 -> e_1 )( \tau _2 -> e_2 ) \dots  
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(e \phiTerminal{(} \tau _1 \mathbin{\phiTerminal{\mapsto}} e_1 \phiTerminal{)}\phiTerminal{(} \tau _2 \mathbin{\phiTerminal{\mapsto}} e_2 \phiTerminal{)} \dots\)\endinput

==> _eolang/paper/9FBFA353E4EA74C38ACA4A758EB912D4-58-phiq.tex <==
 e ( \tau _1 -> e_1 )( \tau _2 -> e_2 ) \dots  

==> _eolang/paper/A2AA7586B12853D6E58E4D8D440C485A-19-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 11 chars in the input: _eolang/paper/A2AA7586B12853D6E58E4D8D440C485A-19-phiq.tex
% ---
% n = [[ B ]]
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(n = \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/A2AA7586B12853D6E58E4D8D440C485A-19-phiq.tex <==
n = [[ B ]]

==> _eolang/paper/A2AA7586B12853D6E58E4D8D440C485A-22-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 11 chars in the input: _eolang/paper/A2AA7586B12853D6E58E4D8D440C485A-22-phiq.tex
% ---
% n = [[ B ]]
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(n = \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/A2AA7586B12853D6E58E4D8D440C485A-22-phiq.tex <==
n = [[ B ]]

==> _eolang/paper/A4373A694CE7D6CD9DCC81E8E71B96E3-13-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 53 chars in the input: _eolang/paper/A4373A694CE7D6CD9DCC81E8E71B96E3-13-phiq.tex
% ---
%  [ L ] \cap \lparen B_1 \cup B_2 \rparen = \emptyset 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\([ \phiTerminal{\uplambda{}} ] \cap \lparen B_1 \cup B_2 \rparen = \emptyset\)\endinput

==> _eolang/paper/A4373A694CE7D6CD9DCC81E8E71B96E3-13-phiq.tex <==
 [ L ] \cap \lparen B_1 \cup B_2 \rparen = \emptyset 

==> _eolang/paper/A50F3D3616FDF47BE56E5459434BE9E6-60-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 39 chars in the input: _eolang/paper/A50F3D3616FDF47BE56E5459434BE9E6-60-phiq.tex
% ---
% \phinoNormalize { [[ B ]] . \tau }{ T }
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} \phiTerminal{.} \tau }{  \phiTerminal{\bot{}} }\)\endinput

==> _eolang/paper/A50F3D3616FDF47BE56E5459434BE9E6-60-phiq.tex <==
\phinoNormalize { [[ B ]] . \tau }{ T }

==> _eolang/paper/A58356E6D3C5695FC38AD8821791EB76-35-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 45 chars in the input: _eolang/paper/A58356E6D3C5695FC38AD8821791EB76-35-phiq.tex
% ---
% \phiText {if}  \phiTerminal {\rho } \notin B 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiText {if}  \phiTerminal {\uprho } \notin B\)\endinput

==> _eolang/paper/A58356E6D3C5695FC38AD8821791EB76-35-phiq.tex <==
\phiText {if}  \phiTerminal {\rho } \notin B 

==> _eolang/paper/A58356E6D3C5695FC38AD8821791EB76-50-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 45 chars in the input: _eolang/paper/A58356E6D3C5695FC38AD8821791EB76-50-phiq.tex
% ---
% \phiText {if}  \phiTerminal {\rho } \notin B 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiText {if}  \phiTerminal {\uprho } \notin B\)\endinput

==> _eolang/paper/A58356E6D3C5695FC38AD8821791EB76-50-phiq.tex <==
\phiText {if}  \phiTerminal {\rho } \notin B 

==> _eolang/paper/A5855048483C40E8FFEAC0646476F178-6-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 11 chars in the input: _eolang/paper/A5855048483C40E8FFEAC0646476F178-6-phiq.tex
% ---
% \Downarrow 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\Downarrow\)\endinput

==> _eolang/paper/A5855048483C40E8FFEAC0646476F178-6-phiq.tex <==
\Downarrow 

==> _eolang/paper/A6046DE936BF702246413BAC77962D89-60-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 69 chars in the input: _eolang/paper/A6046DE936BF702246413BAC77962D89-60-phiq.tex
% ---
% \phiText {if}  [ \tau \char 44{} @ \char 44{} L ] \cap B = \emptyset 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiText {if}  [ \tau \char 44{} \phiTerminal{\upvarphi{}} \char 44{} \phiTerminal{\uplambda{}} ] \cap B = \emptyset\)\endinput

==> _eolang/paper/A6046DE936BF702246413BAC77962D89-60-phiq.tex <==
\phiText {if}  [ \tau \char 44{} @ \char 44{} L ] \cap B = \emptyset 

==> _eolang/paper/AA180E751A597A3D01BAD16B810C44C4-64-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 42 chars in the input: _eolang/paper/AA180E751A597A3D01BAD16B810C44C4-64-phiq.tex
% ---
%  \tau _1 -> \phiTerminal {\upxi }.\tau _2 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\tau _1 \mathbin{\phiTerminal{\mapsto}} \phiTerminal {\upxi }\phiTerminal{.}\tau _2\)\endinput

==> _eolang/paper/AA180E751A597A3D01BAD16B810C44C4-64-phiq.tex <==
 \tau _1 -> \phiTerminal {\upxi }.\tau _2 

==> _eolang/paper/ABAD46A2735921BFEA5385EA2C9267B7-7-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 50 chars in the input: _eolang/paper/ABAD46A2735921BFEA5385EA2C9267B7-7-phiq.tex
% ---
%  \phinoDataize { n }{ e }{ s_1 }{ \delta }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoDataize { n }{ e }{ s_1 }{ \delta }{ s_2 }\)\endinput

==> _eolang/paper/ABAD46A2735921BFEA5385EA2C9267B7-7-phiq.tex <==
 \phinoDataize { n }{ e }{ s_1 }{ \delta }{ s_2 } 

==> _eolang/paper/AC2E85E7F45F0A3591422197E8ED4D44-25-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 91 chars in the input: _eolang/paper/AC2E85E7F45F0A3591422197E8ED4D44-25-phiq.tex
% ---
% \phinoNormalize { [[ B_1, \tau -> n, B_2 ]] . \tau }{ e_1 ( \phiTerminal {\rho } -> e_2 ) }
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \tau \mathbin{\phiTerminal{\mapsto}} n\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} \phiTerminal{.} \tau }{ e_1 \phiTerminal{(} \phiTerminal {\uprho } \mathbin{\phiTerminal{\mapsto}} e_2 \phiTerminal{)} }\)\endinput

==> _eolang/paper/AC2E85E7F45F0A3591422197E8ED4D44-25-phiq.tex <==
\phinoNormalize { [[ B_1, \tau -> n, B_2 ]] . \tau }{ e_1 ( \phiTerminal {\rho } -> e_2 ) }

==> _eolang/paper/AC32A7EFBCE3EA8A19C9547F6AAC2373-82-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 76 chars in the input: _eolang/paper/AC32A7EFBCE3EA8A19C9547F6AAC2373-82-phiq.tex
% ---
%   Q.|number| ( @ -> Q.|bytes| ( @ -> [[ D> |7F-F8-00-00-00-00-00-00| ]] ) ) 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{number}}{} \phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}}  \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{bytes}}{} \phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{7F-F8-00-00-00-00-00-00}}{} \phiTerminal{\rrbracket{}} \phiTerminal{)} \phiTerminal{)}\)\endinput

==> _eolang/paper/AC32A7EFBCE3EA8A19C9547F6AAC2373-82-phiq.tex <==
  Q.|number| ( @ -> Q.|bytes| ( @ -> [[ D> |7F-F8-00-00-00-00-00-00| ]] ) ) 

==> _eolang/paper/ACD2217CFF242B675FC1DAC72D31D0D7-24-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 334 chars in the input: _eolang/paper/ACD2217CFF242B675FC1DAC72D31D0D7-24-phiquation.tex
% ---
% [[ |x| -> ?, |y| -> |x| ]] ( |x| -> |42.0| ) . |y| \phiNormalize[\nameref{r:copy}]
%   \phiNormalize \phinoMeet{basic-f:1}{ [[ |x| -> |42.0|, |y| -> |x| ]] } . |y| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize |42.0| : |x| . |x| ( \phiTerminal{\rho} -> \phinoAgain{basic-f:1} ) \phiNormalize[\nameref{r:dot}]
%   \phiNormalize |42.0|{.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}}\phiTerminal{,}\; \textnormal{\texttt{y}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{x}}{} \phiTerminal{\rrbracket{}} \phiTerminal{(} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{)} \phiTerminal{.} \textnormal{\texttt{y}}{} \phiNormalize[\nameref{r:copy}]\phiEOL{}
& \quad{}\phiNormalize \phinoMeet{basic-f:1}{ \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{}\phiTerminal{,}\; \textnormal{\texttt{y}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{x}}{} \phiTerminal{\rrbracket{}} } \phiTerminal{.} \textnormal{\texttt{y}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \textnormal{\texttt{42.0}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{x}}{} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-f:1} \phiTerminal{)} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \textnormal{\texttt{42.0}}{}{.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/ACD2217CFF242B675FC1DAC72D31D0D7-24-phiquation.tex <==
[[ |x| -> ?, |y| -> |x| ]] ( |x| -> |42.0| ) . |y| \phiNormalize[\nameref{r:copy}]
  \phiNormalize \phinoMeet{basic-f:1}{ [[ |x| -> |42.0|, |y| -> |x| ]] } . |y| \phiNormalize[\nameref{r:dot}]
  \phiNormalize |42.0| : |x| . |x| ( \phiTerminal{\rho} -> \phinoAgain{basic-f:1} ) \phiNormalize[\nameref{r:dot}]
  \phiNormalize |42.0|{.}


==> _eolang/paper/ADEE64C160F0FE22B2A161E0C201DB60-40-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 57 chars in the input: _eolang/paper/ADEE64C160F0FE22B2A161E0C201DB60-40-phiq.tex
% ---
% \phinoNormalize { [[ B_1, \tau -> ?, B_2 ]] . \tau }{ T }
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \tau \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}}\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} \phiTerminal{.} \tau }{  \phiTerminal{\bot{}} }\)\endinput

==> _eolang/paper/ADEE64C160F0FE22B2A161E0C201DB60-40-phiq.tex <==
\phinoNormalize { [[ B_1, \tau -> ?, B_2 ]] . \tau }{ T }

==> _eolang/paper/B21CF7BEA1057351558F451BC2B2BC10-53-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 34 chars in the input: _eolang/paper/B21CF7BEA1057351558F451BC2B2BC10-53-phiq.tex
% ---
% \phinoEvaluate {b}{e}{s}{ n_3 }{s}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoEvaluate {b}{e}{s}{ n_3 }{s}\)\endinput

==> _eolang/paper/B21CF7BEA1057351558F451BC2B2BC10-53-phiq.tex <==
\phinoEvaluate {b}{e}{s}{ n_3 }{s}

==> _eolang/paper/B3186FD7F04BC039AC5DBB0625A6D893-22-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 5 chars in the input: _eolang/paper/B3186FD7F04BC039AC5DBB0625A6D893-22-phiq.tex
% ---
% e = Q
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(e =  \phiTerminal{\Phi{}}\)\endinput

==> _eolang/paper/B3186FD7F04BC039AC5DBB0625A6D893-22-phiq.tex <==
e = Q

==> _eolang/paper/B6F9E8410132DA8B94681FC2D13763D9-10-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 5 chars in the input: _eolang/paper/B6F9E8410132DA8B94681FC2D13763D9-10-phiq.tex
% ---
% n = T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(n =  \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B6F9E8410132DA8B94681FC2D13763D9-10-phiq.tex <==
n = T

==> _eolang/paper/B6F9E8410132DA8B94681FC2D13763D9-16-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 5 chars in the input: _eolang/paper/B6F9E8410132DA8B94681FC2D13763D9-16-phiq.tex
% ---
% n = T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(n =  \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B6F9E8410132DA8B94681FC2D13763D9-16-phiq.tex <==
n = T

==> _eolang/paper/B7A1E2488E11827E2862847BF0049C9E-53-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 35 chars in the input: _eolang/paper/B7A1E2488E11827E2862847BF0049C9E-53-phiq.tex
% ---
% \delta = \delta _1 \times \delta _2
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\delta = \delta _1 \times \delta _2\)\endinput

==> _eolang/paper/B7A1E2488E11827E2862847BF0049C9E-53-phiq.tex <==
\delta = \delta _1 \times \delta _2

==> _eolang/paper/B7B3918C74D72DA8B7AF54807E8F127B-175-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 12 chars in the input: _eolang/paper/B7B3918C74D72DA8B7AF54807E8F127B-175-phiq.tex
% ---
% Q.|k|.|next|
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{k}}{}\phiTerminal{.}\textnormal{\texttt{next}}{}\)\endinput

==> _eolang/paper/B7B3918C74D72DA8B7AF54807E8F127B-175-phiq.tex <==
Q.|k|.|next|

==> _eolang/paper/B7CE5ED9F5DED23AB56F4BB3F8695658-23-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 37 chars in the input: _eolang/paper/B7CE5ED9F5DED23AB56F4BB3F8695658-23-phiq.tex
% ---
%  \phinoContextualize { T }{ k }{ T } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoContextualize {  \phiTerminal{\bot{}} }{ k }{  \phiTerminal{\bot{}} }\)\endinput

==> _eolang/paper/B7CE5ED9F5DED23AB56F4BB3F8695658-23-phiq.tex <==
 \phinoContextualize { T }{ k }{ T } 

==> _eolang/paper/B8D4DB288BCEAD45982CBDBF208A5D83-17-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 31 chars in the input: _eolang/paper/B8D4DB288BCEAD45982CBDBF208A5D83-17-phiq.tex
% ---
% [[ B_1, \tau -> n, B_2 ]].\tau 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\llbracket} B_1\phiTerminal{,}\; \tau \mathbin{\phiTerminal{\mapsto}} n\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}}\phiTerminal{.}\tau\)\endinput

==> _eolang/paper/B8D4DB288BCEAD45982CBDBF208A5D83-17-phiq.tex <==
[[ B_1, \tau -> n, B_2 ]].\tau 

==> _eolang/paper/B91C7FB1D367207DE7C636C9437DEA65-5-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 88 chars in the input: _eolang/paper/B91C7FB1D367207DE7C636C9437DEA65-5-phiq.tex
% ---
% \phinoNormalize { [[ B_1, \tau -> ?, B_2 ]] ( \tau -> k ) }{ [[ B_1, \tau -> k, B_2 ]] }
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \tau \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}}\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} \phiTerminal{(} \tau \mathbin{\phiTerminal{\mapsto}} k \phiTerminal{)} }{ \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \tau \mathbin{\phiTerminal{\mapsto}} k\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} }\)\endinput

==> _eolang/paper/B91C7FB1D367207DE7C636C9437DEA65-5-phiq.tex <==
\phinoNormalize { [[ B_1, \tau -> ?, B_2 ]] ( \tau -> k ) }{ [[ B_1, \tau -> k, B_2 ]] }

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-102-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-102-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-102-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-11-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-11-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-11-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-12-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-12-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-12-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-13-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-13-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-13-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-14-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-14-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-14-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-15-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-15-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-15-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-17-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-17-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-17-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-177-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-177-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-177-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-18-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-18-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-18-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-181-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-181-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-181-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-19-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-19-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-19-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-203-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-203-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-203-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-222-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-222-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-222-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-223-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-223-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-223-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-30-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-30-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-30-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-31-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-31-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-31-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-33-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-33-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-33-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-36-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-36-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-36-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-42-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-42-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-42-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-43-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-43-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-43-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-47-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-47-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-47-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-52-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-52-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-52-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-57-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-57-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-57-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-6-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-6-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-6-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-8-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-8-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-8-phiq.tex <==
T

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-9-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-9-phiq.tex
% ---
% T
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\bot{}}\)\endinput

==> _eolang/paper/B9ECE18C950AFBFA6B0FDBFA4FF731D3-9-phiq.tex <==
T

==> _eolang/paper/BB7522BD098ABC5E1BB37D9DDF9FBE2E-20-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 56 chars in the input: _eolang/paper/BB7522BD098ABC5E1BB37D9DDF9FBE2E-20-phiq.tex
% ---
%  \phinoDataize { [[ B ]] }{ e }{ s_1 }{ \delta }{ s_3 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoDataize { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} }{ e }{ s_1 }{ \delta }{ s_3 }\)\endinput

==> _eolang/paper/BB7522BD098ABC5E1BB37D9DDF9FBE2E-20-phiq.tex <==
 \phinoDataize { [[ B ]] }{ e }{ s_1 }{ \delta }{ s_3 } 

==> _eolang/paper/BDF4A8F896ECF97EDF870197A7B3B380-7-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 62 chars in the input: _eolang/paper/BDF4A8F896ECF97EDF870197A7B3B380-7-phiq.tex
% ---
%  @ \in B \phiText {and} [ D \char 44{} L ] \cap B = \emptyset 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\upvarphi{}} \in B \phiText {and} [ \phiTerminal{\Delta{}} \char 44{} \phiTerminal{\uplambda{}} ] \cap B = \emptyset\)\endinput

==> _eolang/paper/BDF4A8F896ECF97EDF870197A7B3B380-7-phiq.tex <==
 @ \in B \phiText {and} [ D \char 44{} L ] \cap B = \emptyset 

==> _eolang/paper/BE601A88FB734B2FC0E6B4D360F58A0F-9-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 29 chars in the input: _eolang/paper/BE601A88FB734B2FC0E6B4D360F58A0F-9-phiquation.tex
% ---
% [[ |x| -> |t|, L> |Fn| ]]{.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{t}}{}\phiTerminal{,}\; \phiTerminal{\uplambda{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{Fn}}{} \phiTerminal{\rrbracket{}}{.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/BE601A88FB734B2FC0E6B4D360F58A0F-9-phiquation.tex <==
[[ |x| -> |t|, L> |Fn| ]]{.}


==> _eolang/paper/C00EC321363A8998E8DADBC71A502620-18-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 9 chars in the input: _eolang/paper/C00EC321363A8998E8DADBC71A502620-18-phiq.tex
% ---
% e_1.\tau 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(e_1\phiTerminal{.}\tau\)\endinput

==> _eolang/paper/C00EC321363A8998E8DADBC71A502620-18-phiq.tex <==
e_1.\tau 

==> _eolang/paper/C3DF7C36E97255B3ACC4E0FB1E822E3A-65-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 43 chars in the input: _eolang/paper/C3DF7C36E97255B3ACC4E0FB1E822E3A-65-phiq.tex
% ---
%  \phinoMorph { T }{ e }{ s_1 }{ n }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph {  \phiTerminal{\bot{}} }{ e }{ s_1 }{ n }{ s_2 }\)\endinput

==> _eolang/paper/C3DF7C36E97255B3ACC4E0FB1E822E3A-65-phiq.tex <==
 \phinoMorph { T }{ e }{ s_1 }{ n }{ s_2 } 

==> _eolang/paper/C5C6FFCB5E3F188410DF1CCB1880F095-47-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 437 chars in the input: _eolang/paper/C5C6FFCB5E3F188410DF1CCB1880F095-47-phiquation.tex
% ---
% [[ |x| -> [[ \phiTerminal{\rho} -> ? ]] . \phiTerminal{\rho} . |k|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:null}]
%   \phiNormalize [[ |x| -> T . |k|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dd}]
%   \phiNormalize \phinoMeet{basic-j:1}{ [[ |x| -> T, |k| -> |42.0| ]] } . |x| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize T ( \phiTerminal{\rho} -> \phinoAgain{basic-j:1} ) \phiNormalize[\nameref{r:dc}]
%   \phiNormalize T{.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}} \phiTerminal{\rrbracket{}} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{k}}{}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:null}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\bot{}} \phiTerminal{.} \textnormal{\texttt{k}}{}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dd}]\phiEOL{}
& \quad{}\phiNormalize \phinoMeet{basic-j:1}{ \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\bot{}}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} } \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-j:1} \phiTerminal{)} \phiNormalize[\nameref{r:dc}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}}{.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/C5C6FFCB5E3F188410DF1CCB1880F095-47-phiquation.tex <==
[[ |x| -> [[ \phiTerminal{\rho} -> ? ]] . \phiTerminal{\rho} . |k|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:null}]
  \phiNormalize [[ |x| -> T . |k|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dd}]
  \phiNormalize \phinoMeet{basic-j:1}{ [[ |x| -> T, |k| -> |42.0| ]] } . |x| \phiNormalize[\nameref{r:dot}]
  \phiNormalize T ( \phiTerminal{\rho} -> \phinoAgain{basic-j:1} ) \phiNormalize[\nameref{r:dc}]
  \phiNormalize T{.}


==> _eolang/paper/C62834CF47380CB628B682E703EC7FCE-57-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 941 chars in the input: _eolang/paper/C62834CF47380CB628B682E703EC7FCE-57-phiquation.tex
% ---
% \phinoMeet{basic-k:1}{ [[ |x| -> |t| ( |k| -> [[]] ) . |k|, |t|(|k|) -> [[]] ]] } . |x| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize [[ |t|(|k|) -> [[]] ]] . |t| ( |k| -> [[]] ) . |k| ( \phiTerminal{\rho} -> \phinoAgain{basic-k:1} ) \phiNormalize[\nameref{r:dot}]
%   \phiNormalize ? : |k| ( \phiTerminal{\rho} -> [[ |t|(|k|) -> [[]] ]], |k| -> [[]] ) . |k| ( \phiTerminal{\rho} -> \phinoAgain{basic-k:1} ) \phiNormalize[\nameref{r:skip}]
%   \phiNormalize ? : |k| ( |k| -> [[]] ) . |k| ( \phiTerminal{\rho} -> \phinoAgain{basic-k:1} ) \phiNormalize[\nameref{r:copy}]
%   \phiNormalize [[]] : |k| . |k| ( \phiTerminal{\rho} -> \phinoAgain{basic-k:1} ) \phiNormalize[\nameref{r:dot}]
%   \phiNormalize [[]] ( \phiTerminal{\rho} -> [[]] : |k|, \phiTerminal{\rho} -> \phinoAgain{basic-k:1} ) \phiNormalize[\nameref{r:skip}]
%   \phiNormalize [[]] ( \phiTerminal{\rho} -> \phinoAgain{basic-k:1} ) \phiNormalize[\nameref{r:skip}]
%   \phiNormalize [[]]{.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phinoMeet{basic-k:1}{ \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{t}}{} \phiTerminal{(} \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{)} \phiTerminal{.} \textnormal{\texttt{k}}{}\phiTerminal{,}\; \textnormal{\texttt{t}}{}\phiTerminal{(}\textnormal{\texttt{k}}{}\phiTerminal{)} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}} } \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{t}}{}\phiTerminal{(}\textnormal{\texttt{k}}{}\phiTerminal{)} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{(} \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{)} \phiTerminal{.} \textnormal{\texttt{k}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-k:1} \phiTerminal{)} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\varnothing{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{k}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \textnormal{\texttt{t}}{}\phiTerminal{(}\textnormal{\texttt{k}}{}\phiTerminal{)} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{\rrbracket{}}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{)} \phiTerminal{.} \textnormal{\texttt{k}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-k:1} \phiTerminal{)} \phiNormalize[\nameref{r:skip}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\varnothing{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{k}}{} \phiTerminal{(} \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{)} \phiTerminal{.} \textnormal{\texttt{k}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-k:1} \phiTerminal{)} \phiNormalize[\nameref{r:copy}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{k}}{} \phiTerminal{.} \textnormal{\texttt{k}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-k:1} \phiTerminal{)} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{k}}{}\phiTerminal{,}\; \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-k:1} \phiTerminal{)} \phiNormalize[\nameref{r:skip}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-k:1} \phiTerminal{)} \phiNormalize[\nameref{r:skip}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}}{.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/C62834CF47380CB628B682E703EC7FCE-57-phiquation.tex <==
\phinoMeet{basic-k:1}{ [[ |x| -> |t| ( |k| -> [[]] ) . |k|, |t|(|k|) -> [[]] ]] } . |x| \phiNormalize[\nameref{r:dot}]
  \phiNormalize [[ |t|(|k|) -> [[]] ]] . |t| ( |k| -> [[]] ) . |k| ( \phiTerminal{\rho} -> \phinoAgain{basic-k:1} ) \phiNormalize[\nameref{r:dot}]
  \phiNormalize ? : |k| ( \phiTerminal{\rho} -> [[ |t|(|k|) -> [[]] ]], |k| -> [[]] ) . |k| ( \phiTerminal{\rho} -> \phinoAgain{basic-k:1} ) \phiNormalize[\nameref{r:skip}]
  \phiNormalize ? : |k| ( |k| -> [[]] ) . |k| ( \phiTerminal{\rho} -> \phinoAgain{basic-k:1} ) \phiNormalize[\nameref{r:copy}]
  \phiNormalize [[]] : |k| . |k| ( \phiTerminal{\rho} -> \phinoAgain{basic-k:1} ) \phiNormalize[\nameref{r:dot}]
  \phiNormalize [[]] ( \phiTerminal{\rho} -> [[]] : |k|, \phiTerminal{\rho} -> \phinoAgain{basic-k:1} ) \phiNormalize[\nameref{r:skip}]
  \phiNormalize [[]] ( \phiTerminal{\rho} -> \phinoAgain{basic-k:1} ) \phiNormalize[\nameref{r:skip}]
  \phiNormalize [[]]{.}


==> _eolang/paper/C6E1AB450B25D895ACAF2C1EDC347F6D-27-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 26 chars in the input: _eolang/paper/C6E1AB450B25D895ACAF2C1EDC347F6D-27-phiq.tex
% ---
% [D, L] \cap B = \emptyset 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\([\phiTerminal{\Delta{}}\phiTerminal{,}\; \phiTerminal{\uplambda{}}] \cap B = \emptyset\)\endinput

==> _eolang/paper/C6E1AB450B25D895ACAF2C1EDC347F6D-27-phiq.tex <==
[D, L] \cap B = \emptyset 

==> _eolang/paper/C6E1AB450B25D895ACAF2C1EDC347F6D-28-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 26 chars in the input: _eolang/paper/C6E1AB450B25D895ACAF2C1EDC347F6D-28-phiq.tex
% ---
% [D, L] \cap B = \emptyset 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\([\phiTerminal{\Delta{}}\phiTerminal{,}\; \phiTerminal{\uplambda{}}] \cap B = \emptyset\)\endinput

==> _eolang/paper/C6E1AB450B25D895ACAF2C1EDC347F6D-28-phiq.tex <==
[D, L] \cap B = \emptyset 

==> _eolang/paper/C7B686893257C698B3E518972553DE3C-270-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 71 chars in the input: _eolang/paper/C7B686893257C698B3E518972553DE3C-270-phiquation.tex
% ---
% e_1 = [[ foo -> ?, D> 01-02 ]] \quad e_2 = [[ bar -> ?, D> 01-02 ]]{.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
e_1 = \phiTerminal{\llbracket} \textnormal{\texttt{foo}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}}\phiTerminal{,}\; \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{01-02}}{} \phiTerminal{\rrbracket{}} \quad e_2 = \phiTerminal{\llbracket} \textnormal{\texttt{bar}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}}\phiTerminal{,}\; \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{01-02}}{} \phiTerminal{\rrbracket{}}{.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/C7B686893257C698B3E518972553DE3C-270-phiquation.tex <==
e_1 = [[ foo -> ?, D> 01-02 ]] \quad e_2 = [[ bar -> ?, D> 01-02 ]]{.}


==> _eolang/paper/C8C2A8C647E8ED4998BF5BAB80C3E7E8-13-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 7 chars in the input: _eolang/paper/C8C2A8C647E8ED4998BF5BAB80C3E7E8-13-phiq.tex
% ---
% [[ B ]]
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/C8C2A8C647E8ED4998BF5BAB80C3E7E8-13-phiq.tex <==
[[ B ]]

==> _eolang/paper/C8C2A8C647E8ED4998BF5BAB80C3E7E8-23-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 7 chars in the input: _eolang/paper/C8C2A8C647E8ED4998BF5BAB80C3E7E8-23-phiq.tex
% ---
% [[ B ]]
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/C8C2A8C647E8ED4998BF5BAB80C3E7E8-23-phiq.tex <==
[[ B ]]

==> _eolang/paper/C8C2A8C647E8ED4998BF5BAB80C3E7E8-74-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 7 chars in the input: _eolang/paper/C8C2A8C647E8ED4998BF5BAB80C3E7E8-74-phiq.tex
% ---
% [[ B ]]
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/C8C2A8C647E8ED4998BF5BAB80C3E7E8-74-phiq.tex <==
[[ B ]]

==> _eolang/paper/C9132881BB077425AF79A085F04F3371-34-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 80 chars in the input: _eolang/paper/C9132881BB077425AF79A085F04F3371-34-phiquation.tex
% ---
% [[ |x| -> ?, |y| -> ? ]]( |x| -> b ) \phiNormalize [[ |x| -> b, |y| -> ? ]] {.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}}\phiTerminal{,}\; \textnormal{\texttt{y}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}} \phiTerminal{\rrbracket{}}\phiTerminal{(} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} b \phiTerminal{)} \phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} b\phiTerminal{,}\; \textnormal{\texttt{y}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}} \phiTerminal{\rrbracket{}} {.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/C9132881BB077425AF79A085F04F3371-34-phiquation.tex <==
[[ |x| -> ?, |y| -> ? ]]( |x| -> b ) \phiNormalize [[ |x| -> b, |y| -> ? ]] {.}


==> _eolang/paper/C95E3A195319EADC47379EA30D13F2BF-55-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 142 chars in the input: _eolang/paper/C95E3A195319EADC47379EA30D13F2BF-55-phiq.tex
% ---
% \phinoNormalize { [[ B_1, \phiTerminal {\rho } -> e_1, B_2 ]] ( \phiTerminal {\rho } -> e_2 ) }{ [[ B_1, \phiTerminal {\rho } -> e_1, B_2 ]] }
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \phiTerminal {\uprho } \mathbin{\phiTerminal{\mapsto}} e_1\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} \phiTerminal{(} \phiTerminal {\uprho } \mathbin{\phiTerminal{\mapsto}} e_2 \phiTerminal{)} }{ \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \phiTerminal {\uprho } \mathbin{\phiTerminal{\mapsto}} e_1\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} }\)\endinput

==> _eolang/paper/C95E3A195319EADC47379EA30D13F2BF-55-phiq.tex <==
\phinoNormalize { [[ B_1, \phiTerminal {\rho } -> e_1, B_2 ]] ( \phiTerminal {\rho } -> e_2 ) }{ [[ B_1, \phiTerminal {\rho } -> e_1, B_2 ]] }

==> _eolang/paper/C9DCFAEEE2E6BA034B055F0CD6E074DD-51-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 47 chars in the input: _eolang/paper/C9DCFAEEE2E6BA034B055F0CD6E074DD-51-phiq.tex
% ---
%  \phinoNormalize { [[ B ]] . @ . \tau }{ n_1 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} \phiTerminal{.} \phiTerminal{\upvarphi{}} \phiTerminal{.} \tau }{ n_1 }\)\endinput

==> _eolang/paper/C9DCFAEEE2E6BA034B055F0CD6E074DD-51-phiq.tex <==
 \phinoNormalize { [[ B ]] . @ . \tau }{ n_1 } 

==> _eolang/paper/CA70D40F9F78FD23E7533D080AFC8B54-45-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 68 chars in the input: _eolang/paper/CA70D40F9F78FD23E7533D080AFC8B54-45-phiq.tex
% ---
% \phinoNormalize { [[ B_1, \tau -> e_1, B_2 ]] ( \tau -> e_2 ) }{ T }
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \tau \mathbin{\phiTerminal{\mapsto}} e_1\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} \phiTerminal{(} \tau \mathbin{\phiTerminal{\mapsto}} e_2 \phiTerminal{)} }{  \phiTerminal{\bot{}} }\)\endinput

==> _eolang/paper/CA70D40F9F78FD23E7533D080AFC8B54-45-phiq.tex <==
\phinoNormalize { [[ B_1, \tau -> e_1, B_2 ]] ( \tau -> e_2 ) }{ T }

==> _eolang/paper/CBAB6D88D310781AC891170A513313CC-61-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 58 chars in the input: _eolang/paper/CBAB6D88D310781AC891170A513313CC-61-phiq.tex
% ---
%  \tau _1 -> [[ \tau _2 -> ? , \tau _3 -> ? , \dots , B ]] 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\tau _1 \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \tau _2 \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}} \phiTerminal{,}\; \tau _3 \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}} \phiTerminal{,}\; \dots \phiTerminal{,}\; B \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/CBAB6D88D310781AC891170A513313CC-61-phiq.tex <==
 \tau _1 -> [[ \tau _2 -> ? , \tau _3 -> ? , \dots , B ]] 

==> _eolang/paper/CBFBB9372422BE33DB1F830A9D93B7E8-155-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 26 chars in the input: _eolang/paper/CBFBB9372422BE33DB1F830A9D93B7E8-155-phiq.tex
% ---
%  \phinoNormalize {e_1}{n} 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize {e_1}{n}\)\endinput

==> _eolang/paper/CBFBB9372422BE33DB1F830A9D93B7E8-155-phiq.tex <==
 \phinoNormalize {e_1}{n} 

==> _eolang/paper/CC0534E85A8CC392A77AA8C581D221E3-95-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 108 chars in the input: _eolang/paper/CC0534E85A8CC392A77AA8C581D221E3-95-phiquation.tex
% ---
% \label{eq:object-example}
%  [[ D> 00-2A, |b| -> b_2(|x| -> b_3).bar, |a| -> [[ L> |Sqrt| ]], foo -> T ]] {.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation}
\begin{split}
&\label{eq:object-example} \phiTerminal{\llbracket} \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{00-2A}}{}\phiTerminal{,}\; \textnormal{\texttt{b}}{} \mathbin{\phiTerminal{\mapsto}} b_2\phiTerminal{(}\textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} b_3\phiTerminal{)}\phiTerminal{.}\textnormal{\texttt{bar}}{}\phiTerminal{,}\; \textnormal{\texttt{a}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\uplambda{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{Sqrt}}{} \phiTerminal{\rrbracket{}}\phiTerminal{,}\; \textnormal{\texttt{foo}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\bot{}} \phiTerminal{\rrbracket{}} {.}
\end{split}
\end{equation}\endinput

==> _eolang/paper/CC0534E85A8CC392A77AA8C581D221E3-95-phiquation.tex <==
\label{eq:object-example}
 [[ D> 00-2A, |b| -> b_2(|x| -> b_3).bar, |a| -> [[ L> |Sqrt| ]], foo -> T ]] {.}


==> _eolang/paper/CD0470D70BD8B0B855C62D25BE06C16B-65-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 61 chars in the input: _eolang/paper/CD0470D70BD8B0B855C62D25BE06C16B-65-phiq.tex
% ---
%  \phinoMorph { \phiTerminal {\xi } }{ e }{ s_1 }{ n }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { \phiTerminal {\upxi } }{ e }{ s_1 }{ n }{ s_2 }\)\endinput

==> _eolang/paper/CD0470D70BD8B0B855C62D25BE06C16B-65-phiq.tex <==
 \phinoMorph { \phiTerminal {\xi } }{ e }{ s_1 }{ n }{ s_2 } 

==> _eolang/paper/CD8AADB38A9EE212F9233177D3C6428C-18-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 417 chars in the input: _eolang/paper/CD8AADB38A9EE212F9233177D3C6428C-18-phiquation.tex
% ---
% [[ |x| -> |Fn| : L . \phiTerminal{\rho} . |k|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:norho}]
%   \phiNormalize [[ |x| -> T . |k|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dd}]
%   \phiNormalize \phinoMeet{basic-e:1}{ [[ |x| -> T, |k| -> |42.0| ]] } . |x| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize T ( \phiTerminal{\rho} -> \phinoAgain{basic-e:1} ) \phiNormalize[\nameref{r:dc}]
%   \phiNormalize T{.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{Fn}}{} \mathord{\phiTerminal{:}} \phiTerminal{\uplambda{}} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{k}}{}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:norho}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\bot{}} \phiTerminal{.} \textnormal{\texttt{k}}{}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dd}]\phiEOL{}
& \quad{}\phiNormalize \phinoMeet{basic-e:1}{ \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\bot{}}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} } \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-e:1} \phiTerminal{)} \phiNormalize[\nameref{r:dc}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}}{.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/CD8AADB38A9EE212F9233177D3C6428C-18-phiquation.tex <==
[[ |x| -> |Fn| : L . \phiTerminal{\rho} . |k|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:norho}]
  \phiNormalize [[ |x| -> T . |k|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dd}]
  \phiNormalize \phinoMeet{basic-e:1}{ [[ |x| -> T, |k| -> |42.0| ]] } . |x| \phiNormalize[\nameref{r:dot}]
  \phiNormalize T ( \phiTerminal{\rho} -> \phinoAgain{basic-e:1} ) \phiNormalize[\nameref{r:dc}]
  \phiNormalize T{.}


==> _eolang/paper/D0E82E8E79443EC41B2180732CA3CC68-53-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 26 chars in the input: _eolang/paper/D0E82E8E79443EC41B2180732CA3CC68-53-phiq.tex
% ---
% \phinoNormalize {b.^}{n_1}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize {b\phiTerminal{.}\phiTerminal{\uprho{}}}{n_1}\)\endinput

==> _eolang/paper/D0E82E8E79443EC41B2180732CA3CC68-53-phiq.tex <==
\phinoNormalize {b.^}{n_1}

==> _eolang/paper/D1457B72C3FB323A2671125AEF3EAB5D-134-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D1457B72C3FB323A2671125AEF3EAB5D-134-phiq.tex
% ---
% ?
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\varnothing{}}\)\endinput

==> _eolang/paper/D1457B72C3FB323A2671125AEF3EAB5D-134-phiq.tex <==
?

==> _eolang/paper/D1457B72C3FB323A2671125AEF3EAB5D-21-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D1457B72C3FB323A2671125AEF3EAB5D-21-phiq.tex
% ---
% ?
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\varnothing{}}\)\endinput

==> _eolang/paper/D1457B72C3FB323A2671125AEF3EAB5D-21-phiq.tex <==
?

==> _eolang/paper/D1457B72C3FB323A2671125AEF3EAB5D-26-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D1457B72C3FB323A2671125AEF3EAB5D-26-phiq.tex
% ---
% ?
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\varnothing{}}\)\endinput

==> _eolang/paper/D1457B72C3FB323A2671125AEF3EAB5D-26-phiq.tex <==
?

==> _eolang/paper/D14F6EBB592A7B3F78EC37D11E2354C7-59-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 30 chars in the input: _eolang/paper/D14F6EBB592A7B3F78EC37D11E2354C7-59-phiq.tex
% ---
%  \phinoNormalize { e }{ n_1 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { e }{ n_1 }\)\endinput

==> _eolang/paper/D14F6EBB592A7B3F78EC37D11E2354C7-59-phiq.tex <==
 \phinoNormalize { e }{ n_1 } 

==> _eolang/paper/D183F7B3DF8D5AB769CEF5DE56F81CAC-43-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 39 chars in the input: _eolang/paper/D183F7B3DF8D5AB769CEF5DE56F81CAC-43-phiq.tex
% ---
%  \phinoNormalize { n_1 . \tau }{ n_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { n_1 \phiTerminal{.} \tau }{ n_2 }\)\endinput

==> _eolang/paper/D183F7B3DF8D5AB769CEF5DE56F81CAC-43-phiq.tex <==
 \phinoNormalize { n_1 . \tau }{ n_2 } 

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-137-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-137-phiq.tex
% ---
% L
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}}\)\endinput

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-137-phiq.tex <==
L

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-147-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-147-phiq.tex
% ---
% L
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}}\)\endinput

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-147-phiq.tex <==
L

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-22-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-22-phiq.tex
% ---
% L
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}}\)\endinput

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-22-phiq.tex <==
L

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-25-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-25-phiq.tex
% ---
% L
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}}\)\endinput

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-25-phiq.tex <==
L

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-28-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-28-phiq.tex
% ---
% L
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}}\)\endinput

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-28-phiq.tex <==
L

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-29-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-29-phiq.tex
% ---
% L
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}}\)\endinput

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-29-phiq.tex <==
L

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-40-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-40-phiq.tex
% ---
% L
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}}\)\endinput

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-40-phiq.tex <==
L

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-41-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-41-phiq.tex
% ---
% L
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}}\)\endinput

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-41-phiq.tex <==
L

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-45-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-45-phiq.tex
% ---
% L
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}}\)\endinput

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-45-phiq.tex <==
L

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-48-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-48-phiq.tex
% ---
% L
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}}\)\endinput

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-48-phiq.tex <==
L

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-61-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-61-phiq.tex
% ---
% L
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}}\)\endinput

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-61-phiq.tex <==
L

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-86-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-86-phiq.tex
% ---
% L
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}}\)\endinput

==> _eolang/paper/D20CAEC3B48A1EEF164CB4CA81BA2587-86-phiq.tex <==
L

==> _eolang/paper/D238FF71A71C65354FDC4AA0A780B949-70-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 28 chars in the input: _eolang/paper/D238FF71A71C65354FDC4AA0A780B949-70-phiq.tex
% ---
% [[ |b| -> e_2, |a| -> e_1 ]]
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\llbracket} \textnormal{\texttt{b}}{} \mathbin{\phiTerminal{\mapsto}} e_2\phiTerminal{,}\; \textnormal{\texttt{a}}{} \mathbin{\phiTerminal{\mapsto}} e_1 \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/D238FF71A71C65354FDC4AA0A780B949-70-phiq.tex <==
[[ |b| -> e_2, |a| -> e_1 ]]

==> _eolang/paper/D2D48064E9FF054773E40B70E7024959-155-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 54 chars in the input: _eolang/paper/D2D48064E9FF054773E40B70E7024959-155-phiq.tex
% ---
%  \phinoEvaluate {[[ B_1, L>f, B_2 ]]}{e}{s_1}{n}{s_2} 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoEvaluate {\phiTerminal{\llbracket} B_1\phiTerminal{,}\; \phiTerminal{\uplambda{}} \mathbin{\phiTerminal{\phiDotted}}f\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}}}{e}{s_1}{n}{s_2}\)\endinput

==> _eolang/paper/D2D48064E9FF054773E40B70E7024959-155-phiq.tex <==
 \phinoEvaluate {[[ B_1, L>f, B_2 ]]}{e}{s_1}{n}{s_2} 

==> _eolang/paper/D61CFDDB3904FF76EDCC8E39D056ED7A-20-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 45 chars in the input: _eolang/paper/D61CFDDB3904FF76EDCC8E39D056ED7A-20-phiq.tex
% ---
% \phinoNormalize { [[ B_1, L> f, B_2 ]] }{ T }
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \phiTerminal{\uplambda{}} \mathbin{\phiTerminal{\phiDotted}} f\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} }{  \phiTerminal{\bot{}} }\)\endinput

==> _eolang/paper/D61CFDDB3904FF76EDCC8E39D056ED7A-20-phiq.tex <==
\phinoNormalize { [[ B_1, L> f, B_2 ]] }{ T }

==> _eolang/paper/D61F187309EDAF69C3EBC5E343771AB7-78-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 16 chars in the input: _eolang/paper/D61F187309EDAF69C3EBC5E343771AB7-78-phiq.tex
% ---
%  \texttt {3.14} 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\texttt {3\phiTerminal{.}14}\)\endinput

==> _eolang/paper/D61F187309EDAF69C3EBC5E343771AB7-78-phiq.tex <==
 \texttt {3.14} 

==> _eolang/paper/D6DDBC862F1A6E81D3BD40DB2D69687F-18-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 23 chars in the input: _eolang/paper/D6DDBC862F1A6E81D3BD40DB2D69687F-18-phiquation.tex
% ---
% Q . |x| : |t| : |x|{.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
 \phiTerminal{\Phi{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{x}}{}{.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/D6DDBC862F1A6E81D3BD40DB2D69687F-18-phiquation.tex <==
Q . |x| : |t| : |x|{.}


==> _eolang/paper/D718B95FCA3812297B2E194BC5CC49B1-7-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 38 chars in the input: _eolang/paper/D718B95FCA3812297B2E194BC5CC49B1-7-phiq.tex
% ---
%  \phinoNormalize { [[ B ]] . @ }{ n } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} \phiTerminal{.} \phiTerminal{\upvarphi{}} }{ n }\)\endinput

==> _eolang/paper/D718B95FCA3812297B2E194BC5CC49B1-7-phiq.tex <==
 \phinoNormalize { [[ B ]] . @ }{ n } 

==> _eolang/paper/D834BB588DF74F4CB31A2EFD7D777C7E-178-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 12 chars in the input: _eolang/paper/D834BB588DF74F4CB31A2EFD7D777C7E-178-phiq.tex
% ---
%  Q.|k|.next 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{k}}{}\phiTerminal{.}\textnormal{\texttt{next}}{}\)\endinput

==> _eolang/paper/D834BB588DF74F4CB31A2EFD7D777C7E-178-phiq.tex <==
 Q.|k|.next 

==> _eolang/paper/D8FF0455B97E8FDBBFDEBDE8F68D7F9E-43-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 9 chars in the input: _eolang/paper/D8FF0455B97E8FDBBFDEBDE8F68D7F9E-43-phiq.tex
% ---
%  L \in B 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}} \in B\)\endinput

==> _eolang/paper/D8FF0455B97E8FDBBFDEBDE8F68D7F9E-43-phiq.tex <==
 L \in B 

==> _eolang/paper/DC216396D888B0199CC662998D1C7620-50-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 68 chars in the input: _eolang/paper/DC216396D888B0199CC662998D1C7620-50-phiq.tex
% ---
% \phinoNormalize { [[ B ]] ( \phiTerminal {\rho } -> e ) }{ [[ B ]] }
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} \phiTerminal{(} \phiTerminal {\uprho } \mathbin{\phiTerminal{\mapsto}} e \phiTerminal{)} }{ \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} }\)\endinput

==> _eolang/paper/DC216396D888B0199CC662998D1C7620-50-phiq.tex <==
\phinoNormalize { [[ B ]] ( \phiTerminal {\rho } -> e ) }{ [[ B ]] }

==> _eolang/paper/DC7524EB699769052FF8A0410771D94E-18-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 14 chars in the input: _eolang/paper/DC7524EB699769052FF8A0410771D94E-18-phiq.tex
% ---
% [[ B_1, B_2 ]]
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\llbracket} B_1\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/DC7524EB699769052FF8A0410771D94E-18-phiq.tex <==
[[ B_1, B_2 ]]

==> _eolang/paper/DC7524EB699769052FF8A0410771D94E-26-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 14 chars in the input: _eolang/paper/DC7524EB699769052FF8A0410771D94E-26-phiq.tex
% ---
% [[ B_1, B_2 ]]
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\llbracket} B_1\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/DC7524EB699769052FF8A0410771D94E-26-phiq.tex <==
[[ B_1, B_2 ]]

==> _eolang/paper/DD04C881C352B277AF041A94DCCA96AC-79-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1347 chars in the input: _eolang/paper/DD04C881C352B277AF041A94DCCA96AC-79-phiquation.tex
% ---
% [[ |x| -> \phiTerminal{\rho} . \phiTerminal{\rho} . |k| : |p| . |p| : |t| . |t|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize [[ |x| -> [[]] . \phiTerminal{\rho} . \phiTerminal{\rho} . |k| ( \phiTerminal{\rho} -> \phiTerminal{\rho} . \phiTerminal{\rho} . |k| : |p| ) : |t| . |t|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:norho}]
%   \phiNormalize [[ |x| -> T . \phiTerminal{\rho} . |k| ( \phiTerminal{\rho} -> \phiTerminal{\rho} . \phiTerminal{\rho} . |k| : |p| ) : |t| . |t|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dd}]
%   \phiNormalize [[ |x| -> T . |k| ( \phiTerminal{\rho} -> \phiTerminal{\rho} . \phiTerminal{\rho} . |k| : |p| ) : |t| . |t|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dd}]
%   \phiNormalize [[ |x| -> T ( \phiTerminal{\rho} -> \phiTerminal{\rho} . \phiTerminal{\rho} . |k| : |p| ) : |t| . |t|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dc}]
%   \phiNormalize [[ |x| -> T : |t| . |t|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize [[ |x| -> T ( \phiTerminal{\rho} -> T : |t| ), |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dc}]
%   \phiNormalize \phinoMeet{basic-m:1}{ [[ |x| -> T, |k| -> |42.0| ]] } . |x| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize T ( \phiTerminal{\rho} -> \phinoAgain{basic-m:1} ) \phiNormalize[\nameref{r:dc}]
%   \phiNormalize T{.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\uprho} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{k}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{p}}{} \phiTerminal{.} \textnormal{\texttt{p}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{.} \textnormal{\texttt{t}}{}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket}\phiTerminal{\rrbracket{}} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{k}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\uprho} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{k}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{p}}{} \phiTerminal{)} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{.} \textnormal{\texttt{t}}{}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:norho}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\bot{}} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{k}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\uprho} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{k}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{p}}{} \phiTerminal{)} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{.} \textnormal{\texttt{t}}{}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dd}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\bot{}} \phiTerminal{.} \textnormal{\texttt{k}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\uprho} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{k}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{p}}{} \phiTerminal{)} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{.} \textnormal{\texttt{t}}{}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dd}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\bot{}} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\uprho} \phiTerminal{.} \phiTerminal{\uprho} \phiTerminal{.} \textnormal{\texttt{k}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{p}}{} \phiTerminal{)} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{.} \textnormal{\texttt{t}}{}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dc}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\bot{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{.} \textnormal{\texttt{t}}{}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\bot{}} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\bot{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{)}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dc}]\phiEOL{}
& \quad{}\phiNormalize \phinoMeet{basic-m:1}{ \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\bot{}}\phiTerminal{,}\; \textnormal{\texttt{k}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}} } \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-m:1} \phiTerminal{)} \phiNormalize[\nameref{r:dc}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}}{.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/DD04C881C352B277AF041A94DCCA96AC-79-phiquation.tex <==
[[ |x| -> \phiTerminal{\rho} . \phiTerminal{\rho} . |k| : |p| . |p| : |t| . |t|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dot}]
  \phiNormalize [[ |x| -> [[]] . \phiTerminal{\rho} . \phiTerminal{\rho} . |k| ( \phiTerminal{\rho} -> \phiTerminal{\rho} . \phiTerminal{\rho} . |k| : |p| ) : |t| . |t|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:norho}]
  \phiNormalize [[ |x| -> T . \phiTerminal{\rho} . |k| ( \phiTerminal{\rho} -> \phiTerminal{\rho} . \phiTerminal{\rho} . |k| : |p| ) : |t| . |t|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dd}]
  \phiNormalize [[ |x| -> T . |k| ( \phiTerminal{\rho} -> \phiTerminal{\rho} . \phiTerminal{\rho} . |k| : |p| ) : |t| . |t|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dd}]
  \phiNormalize [[ |x| -> T ( \phiTerminal{\rho} -> \phiTerminal{\rho} . \phiTerminal{\rho} . |k| : |p| ) : |t| . |t|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dc}]
  \phiNormalize [[ |x| -> T : |t| . |t|, |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dot}]
  \phiNormalize [[ |x| -> T ( \phiTerminal{\rho} -> T : |t| ), |k| -> |42.0| ]] . |x| \phiNormalize[\nameref{r:dc}]
  \phiNormalize \phinoMeet{basic-m:1}{ [[ |x| -> T, |k| -> |42.0| ]] } . |x| \phiNormalize[\nameref{r:dot}]
  \phiNormalize T ( \phiTerminal{\rho} -> \phinoAgain{basic-m:1} ) \phiNormalize[\nameref{r:dc}]
  \phiNormalize T{.}


==> _eolang/paper/DD1A140F8BF751CA19FCFB0E8897983A-19-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 18 chars in the input: _eolang/paper/DD1A140F8BF751CA19FCFB0E8897983A-19-phiq.tex
% ---
% e_1( \tau -> e_2 )
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(e_1\phiTerminal{(} \tau \mathbin{\phiTerminal{\mapsto}} e_2 \phiTerminal{)}\)\endinput

==> _eolang/paper/DD1A140F8BF751CA19FCFB0E8897983A-19-phiq.tex <==
e_1( \tau -> e_2 )

==> _eolang/paper/E0099CB247C64613CBD33560FA5CCCD0-41-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 20 chars in the input: _eolang/paper/E0099CB247C64613CBD33560FA5CCCD0-41-phiq.tex
% ---
% [[ B_1, L> F, B_2 ]]
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\llbracket} B_1\phiTerminal{,}\; \phiTerminal{\uplambda{}} \mathbin{\phiTerminal{\phiDotted}} F\phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/E0099CB247C64613CBD33560FA5CCCD0-41-phiq.tex <==
[[ B_1, L> F, B_2 ]]

==> _eolang/paper/E1405E5FBAACA5E4564CD0AA6D4A1930-99-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 5 chars in the input: _eolang/paper/E1405E5FBAACA5E4564CD0AA6D4A1930-99-phiq.tex
% ---
%  ..> 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\mathbin{\phiTerminal{\phiDotted}}\)\endinput

==> _eolang/paper/E1405E5FBAACA5E4564CD0AA6D4A1930-99-phiq.tex <==
 ..> 

==> _eolang/paper/E1D8FEEECFB3E3C9EBF0B99BD261FF56-56-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 51 chars in the input: _eolang/paper/E1D8FEEECFB3E3C9EBF0B99BD261FF56-56-phiquation.tex
% ---
% [[ |x| -> b_1 ]]( |x| -> b_2 ) \phiNormalize T {.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} b_1 \phiTerminal{\rrbracket{}}\phiTerminal{(} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} b_2 \phiTerminal{)} \phiNormalize \phiTerminal{\bot{}} {.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/E1D8FEEECFB3E3C9EBF0B99BD261FF56-56-phiquation.tex <==
[[ |x| -> b_1 ]]( |x| -> b_2 ) \phiNormalize T {.}


==> _eolang/paper/E7FD918FD72ABC198CEC552532706253-26-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 52 chars in the input: _eolang/paper/E7FD918FD72ABC198CEC552532706253-26-phiq.tex
% ---
%  [ D \char 44{} L \char 44{} @ ] \cap B = \emptyset 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\([ \phiTerminal{\Delta{}} \char 44{} \phiTerminal{\uplambda{}} \char 44{} \phiTerminal{\upvarphi{}} ] \cap B = \emptyset\)\endinput

==> _eolang/paper/E7FD918FD72ABC198CEC552532706253-26-phiq.tex <==
 [ D \char 44{} L \char 44{} @ ] \cap B = \emptyset 

==> _eolang/paper/E8E08AC2AFCFE56398B31823C1DE621D-155-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 22 chars in the input: _eolang/paper/E8E08AC2AFCFE56398B31823C1DE621D-155-phiq.tex
% ---
%  \uplambda \not \in B 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\uplambda \not \in B\)\endinput

==> _eolang/paper/E8E08AC2AFCFE56398B31823C1DE621D-155-phiq.tex <==
 \uplambda \not \in B 

==> _eolang/paper/E9E514CB54AECCF7B69628AB27668862-61-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 52 chars in the input: _eolang/paper/E9E514CB54AECCF7B69628AB27668862-61-phiq.tex
% ---
%  \tau _1 ( \tau _2 ,\; \tau _3 , \dots ) -> [[ B ]] 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\tau _1 \phiTerminal{(} \tau _2 \phiTerminal{,}\;\; \tau _3 \phiTerminal{,}\; \dots \phiTerminal{)} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}}\)\endinput

==> _eolang/paper/E9E514CB54AECCF7B69628AB27668862-61-phiq.tex <==
 \tau _1 ( \tau _2 ,\; \tau _3 , \dots ) -> [[ B ]] 

==> _eolang/paper/ED458EC2FEFA3828574383842486D81B-155-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 45 chars in the input: _eolang/paper/ED458EC2FEFA3828574383842486D81B-155-phiq.tex
% ---
%  \phinoEvaluate {[[ B ]]}{e}{s}{ [[ B ]]}{s} 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoEvaluate {\phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}}}{e}{s}{ \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}}}{s}\)\endinput

==> _eolang/paper/ED458EC2FEFA3828574383842486D81B-155-phiq.tex <==
 \phinoEvaluate {[[ B ]]}{e}{s}{ [[ B ]]}{s} 

==> _eolang/paper/ED90357894F4092415B266D35B7396A3-70-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 70 chars in the input: _eolang/paper/ED90357894F4092415B266D35B7396A3-70-phiq.tex
% ---
%   Q.|string| ( @ -> Q.|bytes| ( @ -> [[ D> |E4-BD-A0-E5-A5-BD| ]] ) ) 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{string}}{} \phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}}  \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{bytes}}{} \phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \textnormal{\texttt{E4-BD-A0-E5-A5-BD}}{} \phiTerminal{\rrbracket{}} \phiTerminal{)} \phiTerminal{)}\)\endinput

==> _eolang/paper/ED90357894F4092415B266D35B7396A3-70-phiq.tex <==
  Q.|string| ( @ -> Q.|bytes| ( @ -> [[ D> |E4-BD-A0-E5-A5-BD| ]] ) ) 

==> _eolang/paper/ED93C7BDEE97624DF31A75A158719EF4-85-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 12 chars in the input: _eolang/paper/ED93C7BDEE97624DF31A75A158719EF4-85-phiq.tex
% ---
%   Q.|pinf|  
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{pinf}}{}\)\endinput

==> _eolang/paper/ED93C7BDEE97624DF31A75A158719EF4-85-phiq.tex <==
  Q.|pinf|  

==> _eolang/paper/EEA05D612412C3849A6F8C37B2313987-11-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 41 chars in the input: _eolang/paper/EEA05D612412C3849A6F8C37B2313987-11-phiq.tex
% ---
%  \phinoContextualize { n_1 }{ k }{ n_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoContextualize { n_1 }{ k }{ n_2 }\)\endinput

==> _eolang/paper/EEA05D612412C3849A6F8C37B2313987-11-phiq.tex <==
 \phinoContextualize { n_1 }{ k }{ n_2 } 

==> _eolang/paper/EEA05D612412C3849A6F8C37B2313987-6-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 41 chars in the input: _eolang/paper/EEA05D612412C3849A6F8C37B2313987-6-phiq.tex
% ---
%  \phinoContextualize { n_1 }{ k }{ n_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoContextualize { n_1 }{ k }{ n_2 }\)\endinput

==> _eolang/paper/EEA05D612412C3849A6F8C37B2313987-6-phiq.tex <==
 \phinoContextualize { n_1 }{ k }{ n_2 } 

==> _eolang/paper/EECE81DDA9EB9BF60E0B5489AA1BBA01-178-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 7 chars in the input: _eolang/paper/EECE81DDA9EB9BF60E0B5489AA1BBA01-178-phiq.tex
% ---
%  Q.|x| 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\phiTerminal{.}\textnormal{\texttt{x}}{}\)\endinput

==> _eolang/paper/EECE81DDA9EB9BF60E0B5489AA1BBA01-178-phiq.tex <==
 Q.|x| 

==> _eolang/paper/F04C12F5D38F3D418A363726670F4E45-11-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 61 chars in the input: _eolang/paper/F04C12F5D38F3D418A363726670F4E45-11-phiq.tex
% ---
%  \phinoMorph { n_1 ( \tau -> k ) }{ e }{ s_1 }{ n_4 }{ s_3 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { n_1 \phiTerminal{(} \tau \mathbin{\phiTerminal{\mapsto}} k \phiTerminal{)} }{ e }{ s_1 }{ n_4 }{ s_3 }\)\endinput

==> _eolang/paper/F04C12F5D38F3D418A363726670F4E45-11-phiq.tex <==
 \phinoMorph { n_1 ( \tau -> k ) }{ e }{ s_1 }{ n_4 }{ s_3 } 

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-13-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-13-phiq.tex
% ---
% Q
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\)\endinput

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-13-phiq.tex <==
Q

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-16-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-16-phiq.tex
% ---
% Q
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\)\endinput

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-16-phiq.tex <==
Q

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-183-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-183-phiq.tex
% ---
% Q
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\)\endinput

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-183-phiq.tex <==
Q

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-21-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-21-phiq.tex
% ---
% Q
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\)\endinput

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-21-phiq.tex <==
Q

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-26-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-26-phiq.tex
% ---
% Q
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\)\endinput

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-26-phiq.tex <==
Q

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-44-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-44-phiq.tex
% ---
% Q
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\)\endinput

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-44-phiq.tex <==
Q

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-8-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-8-phiq.tex
% ---
% Q
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\( \phiTerminal{\Phi{}}\)\endinput

==> _eolang/paper/F09564C9CA56850D4CD6B3319E541AEE-8-phiq.tex <==
Q

==> _eolang/paper/F322C031FF68ADB2E8AF83F7D29383DE-97-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 4 chars in the input: _eolang/paper/F322C031FF68ADB2E8AF83F7D29383DE-97-phiq.tex
% ---
%  -> 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\mathbin{\phiTerminal{\mapsto}}\)\endinput

==> _eolang/paper/F322C031FF68ADB2E8AF83F7D29383DE-97-phiq.tex <==
 -> 

==> _eolang/paper/F40874407CB88796EE01A88B7B758542-30-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 77 chars in the input: _eolang/paper/F40874407CB88796EE01A88B7B758542-30-phiq.tex
% ---
% \phiText {if}  \tau \notin B \phiText {and} \tau \not = \phiTerminal {\rho } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiText {if}  \tau \notin B \phiText {and} \tau \not = \phiTerminal {\uprho }\)\endinput

==> _eolang/paper/F40874407CB88796EE01A88B7B758542-30-phiq.tex <==
\phiText {if}  \tau \notin B \phiText {and} \tau \not = \phiTerminal {\rho } 

==> _eolang/paper/F453E9FEFAE69BC546845078F1707221-28-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 10 chars in the input: _eolang/paper/F453E9FEFAE69BC546845078F1707221-28-phiq.tex
% ---
% L \notin B
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\uplambda{}} \notin B\)\endinput

==> _eolang/paper/F453E9FEFAE69BC546845078F1707221-28-phiq.tex <==
L \notin B

==> _eolang/paper/F5E75ED6852DC9D7D60D6421EA9A9E9D-53-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 75 chars in the input: _eolang/paper/F5E75ED6852DC9D7D60D6421EA9A9E9D-53-phiq.tex
% ---
% \phinoNormalize { e.number( @ -> e.bytes( @ -> [[ D> \delta ]] ) ) }{ n_3 }
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize { e\phiTerminal{.}\textnormal{\texttt{number}}{}\phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} e\phiTerminal{.}\textnormal{\texttt{bytes}}{}\phiTerminal{(} \phiTerminal{\upvarphi{}} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\llbracket} \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \delta \phiTerminal{\rrbracket{}} \phiTerminal{)} \phiTerminal{)} }{ n_3 }\)\endinput

==> _eolang/paper/F5E75ED6852DC9D7D60D6421EA9A9E9D-53-phiq.tex <==
\phinoNormalize { e.number( @ -> e.bytes( @ -> [[ D> \delta ]] ) ) }{ n_3 }

==> _eolang/paper/F61685EA8240E3F68183A1C7ECF06DED-13-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 71 chars in the input: _eolang/paper/F61685EA8240E3F68183A1C7ECF06DED-13-phiq.tex
% ---
%  \phinoDataize { [[ B_1, D> \delta , B_2 ]] }{ e }{ s }{ \delta }{ s } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoDataize { \phiTerminal{\llbracket} B_1\phiTerminal{,}\; \phiTerminal{\Delta{}} \mathbin{\phiTerminal{\phiDotted}} \delta \phiTerminal{,}\; B_2 \phiTerminal{\rrbracket{}} }{ e }{ s }{ \delta }{ s }\)\endinput

==> _eolang/paper/F61685EA8240E3F68183A1C7ECF06DED-13-phiq.tex <==
 \phinoDataize { [[ B_1, D> \delta , B_2 ]] }{ e }{ s }{ \delta }{ s } 

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-152-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-152-phiq.tex
% ---
% D
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\Delta{}}\)\endinput

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-152-phiq.tex <==
D

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-18-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-18-phiq.tex
% ---
% D
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\Delta{}}\)\endinput

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-18-phiq.tex <==
D

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-216-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-216-phiq.tex
% ---
% D
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\Delta{}}\)\endinput

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-216-phiq.tex <==
D

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-22-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-22-phiq.tex
% ---
% D
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\Delta{}}\)\endinput

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-22-phiq.tex <==
D

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-24-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-24-phiq.tex
% ---
% D
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\Delta{}}\)\endinput

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-24-phiq.tex <==
D

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-28-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-28-phiq.tex
% ---
% D
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\Delta{}}\)\endinput

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-28-phiq.tex <==
D

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-60-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-60-phiq.tex
% ---
% D
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\Delta{}}\)\endinput

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-60-phiq.tex <==
D

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-80-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-80-phiq.tex
% ---
% D
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\Delta{}}\)\endinput

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-80-phiq.tex <==
D

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-97-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 1 chars in the input: _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-97-phiq.tex
% ---
% D
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiTerminal{\Delta{}}\)\endinput

==> _eolang/paper/F623E75AF30E62BBD73D6DF5B50BB7B5-97-phiq.tex <==
D

==> _eolang/paper/F880AD0D2920B7D8DD7DA45B2776A9AA-15-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 33 chars in the input: _eolang/paper/F880AD0D2920B7D8DD7DA45B2776A9AA-15-phiq.tex
% ---
% \phinoNormalize { T . \tau }{ T }
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoNormalize {  \phiTerminal{\bot{}} \phiTerminal{.} \tau }{  \phiTerminal{\bot{}} }\)\endinput

==> _eolang/paper/F880AD0D2920B7D8DD7DA45B2776A9AA-15-phiq.tex <==
\phinoNormalize { T . \tau }{ T }

==> _eolang/paper/F92E7E356DF1981C1E5A27F7623C17D0-17-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 45 chars in the input: _eolang/paper/F92E7E356DF1981C1E5A27F7623C17D0-17-phiq.tex
% ---
%  \phinoMorph { T }{ e }{ s_1 }{ n_2 }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph {  \phiTerminal{\bot{}} }{ e }{ s_1 }{ n_2 }{ s_2 }\)\endinput

==> _eolang/paper/F92E7E356DF1981C1E5A27F7623C17D0-17-phiq.tex <==
 \phinoMorph { T }{ e }{ s_1 }{ n_2 }{ s_2 } 

==> _eolang/paper/F9C03FAB71310FEC06DB34163E3D422E-6-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 318 chars in the input: _eolang/paper/F9C03FAB71310FEC06DB34163E3D422E-6-phiquation.tex
% ---
% \phinoMeet{basic-a:1}{ [[ |x| -> |t|, |t| -> ? ]] } . |x| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize ? : |t| . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-a:1} ) \phiNormalize[\nameref{r:null}]
%   \phiNormalize T ( \phiTerminal{\rho} -> \phinoAgain{basic-a:1} ) \phiNormalize[\nameref{r:dc}]
%   \phiNormalize T{.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phinoMeet{basic-a:1}{ \phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{t}}{}\phiTerminal{,}\; \textnormal{\texttt{t}}{} \mathbin{\phiTerminal{\mapsto}} \phiTerminal{\varnothing{}} \phiTerminal{\rrbracket{}} } \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\varnothing{}} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} \phiTerminal{.} \textnormal{\texttt{t}}{} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-a:1} \phiTerminal{)} \phiNormalize[\nameref{r:null}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}} \phiTerminal{(} \phiTerminal{\uprho} \mathbin{\phiTerminal{\mapsto}} \phinoAgain{basic-a:1} \phiTerminal{)} \phiNormalize[\nameref{r:dc}]\phiEOL{}
& \quad{}\phiNormalize \phiTerminal{\bot{}}{.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/F9C03FAB71310FEC06DB34163E3D422E-6-phiquation.tex <==
\phinoMeet{basic-a:1}{ [[ |x| -> |t|, |t| -> ? ]] } . |x| \phiNormalize[\nameref{r:dot}]
  \phiNormalize ? : |t| . |t| ( \phiTerminal{\rho} -> \phinoAgain{basic-a:1} ) \phiNormalize[\nameref{r:null}]
  \phiNormalize T ( \phiTerminal{\rho} -> \phinoAgain{basic-a:1} ) \phiNormalize[\nameref{r:dc}]
  \phiNormalize T{.}


==> _eolang/paper/FA832DEDC94D496555E40906D9D2655A-20-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 50 chars in the input: _eolang/paper/FA832DEDC94D496555E40906D9D2655A-20-phiq.tex
% ---
% \phiText {if}  D \in \lparen B_1 \cup B_2 \rparen 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phiText {if}  \phiTerminal{\Delta{}} \in \lparen B_1 \cup B_2 \rparen\)\endinput

==> _eolang/paper/FA832DEDC94D496555E40906D9D2655A-20-phiq.tex <==
\phiText {if}  D \in \lparen B_1 \cup B_2 \rparen 

==> _eolang/paper/FBC915A629E5B7713DD3C698C2F03656-51-phiq-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 58 chars in the input: _eolang/paper/FBC915A629E5B7713DD3C698C2F03656-51-phiq.tex
% ---
%  \phinoMorph { [[ B ]] . \tau }{ e }{ s_1 }{ n_2 }{ s_2 } 
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\(\phinoMorph { \phiTerminal{\llbracket} B \phiTerminal{\rrbracket{}} \phiTerminal{.} \tau }{ e }{ s_1 }{ n_2 }{ s_2 }\)\endinput

==> _eolang/paper/FBC915A629E5B7713DD3C698C2F03656-51-phiq.tex <==
 \phinoMorph { [[ B ]] . \tau }{ e }{ s_1 }{ n_2 }{ s_2 } 

==> _eolang/paper/FC817884573F179BE73D5C3C601E4E33-11-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 179 chars in the input: _eolang/paper/FC817884573F179BE73D5C3C601E4E33-11-phiquation.tex
% ---
% \phinoMeet{basic-b:1}{ |42.0| : |t| } . |t| : |x| . |x| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize |42.0| : |x| . |x| \phiNormalize[\nameref{r:dot}]
%   \phiNormalize |42.0|{.}
% ---
% The "gathered" is NOT used because 1 lines are indented
% The "align" is NOT used by default
\begin{equation*}
\begin{split}
&\phinoMeet{basic-b:1}{ \textnormal{\texttt{42.0}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{t}}{} } \phiTerminal{.} \textnormal{\texttt{t}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{x}}{} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \textnormal{\texttt{42.0}}{} \mathord{\phiTerminal{:}} \textnormal{\texttt{x}}{} \phiTerminal{.} \textnormal{\texttt{x}}{} \phiNormalize[\nameref{r:dot}]\phiEOL{}
& \quad{}\phiNormalize \textnormal{\texttt{42.0}}{}{.}
\end{split}
\end{equation*}\endinput

==> _eolang/paper/FC817884573F179BE73D5C3C601E4E33-11-phiquation.tex <==
\phinoMeet{basic-b:1}{ |42.0| : |t| } . |t| : |x| . |x| \phiNormalize[\nameref{r:dot}]
  \phiNormalize |42.0| : |x| . |x| \phiNormalize[\nameref{r:dot}]
  \phiNormalize |42.0|{.}


==> _eolang/paper/FCE4CDCDD6C747E39F16A0FFB320B70E-12-phiquation-post.tex <==
% This file is auto-generated by eolang.sty 0.26.4
% There are 35 chars in the input: _eolang/paper/FCE4CDCDD6C747E39F16A0FFB320B70E-12-phiquation.tex
% ---
% [[ |x| -> |k|, |t| -> |42.0| ]]{.}
% ---
% The "gathered" is used since all lines are left-aligned
% The "align" is NOT used by default
\begin{equation*}
\begin{gathered}
\phiTerminal{\llbracket} \textnormal{\texttt{x}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{k}}{}\phiTerminal{,}\; \textnormal{\texttt{t}}{} \mathbin{\phiTerminal{\mapsto}} \textnormal{\texttt{42.0}}{} \phiTerminal{\rrbracket{}}{.}
\end{gathered}
\end{equation*}\endinput

==> _eolang/paper/FCE4CDCDD6C747E39F16A0FFB320B70E-12-phiquation.tex <==
[[ |x| -> |k|, |t| -> |42.0| ]]{.}


==> _eolang/paper/phiq.tex <==
L

==> _eolang/paper/phiquation.tex <==
\label{eq:celsius}
[[
  @ -> [[ @ -> |c| . |times| ( |x| -> |1.8| ) . |plus| ( |x| -> |32.0| ), |c| -> |25.0| ]],
  |bytes|(@) -> [[]],
  |number|(@) -> [[ |times|(|x|, \phiTerminal{\rho}) -> |Fn1| : L, |plus|(|x|, \phiTerminal{\rho}) -> |Fn2| : L ]]
]]{.}

